Concept-based Explanations for Out-Of-Distribution Detectors

Out-of-distribution (OOD) detection plays a crucial role in ensuring the safe deployment of deep neural network (DNN) classifiers. While a myriad of methods have focused on improving the performance of OOD detectors, a critical gap remains in interpreting their decisions. We help bridge this gap by providing explanations for OOD detectors based on learned high-level concepts. We first propose two new metrics for assessing the effectiveness of a particular set of concepts for explaining OOD detectors: 1) detection completeness, which quantifies the sufficiency of concepts for explaining an OOD-detector's decisions, and 2) concept separability, which captures the distributional separation between in-distribution and OOD data in the concept space. Based on these metrics, we propose an unsupervised framework for learning a set of concepts that satisfy the desired properties of high detection completeness and concept separability, and demonstrate its effectiveness in providing concept-based explanations for diverse off-the-shelf OOD detectors. We also show how to identify prominent concepts contributing to the detection results, and provide further reasoning about their decisions.

==> backups/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> backups/mysymbols.tex <==
% Symbols

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\nmax}{\textnormal{max}}
\newcommand{\nmin}{\textnormal{min}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Tbl.~\ref{#1}}
\newcommand{\eqnref}[1]{Eqn.~(\ref{#1})}
\newcommand{\algref}[1]{Alg.~\ref{#1}}
\newcommand{\thmref}[1]{Thm.~\ref{#1}}
\newcommand{\lemref}[1]{Lem.~\ref{#1}}
\newcommand{\corref}[1]{Cor.~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\propref}[1]{Prop.~\ref{#1}}
\newcommand{\defref}[1]{Def.~\ref{#1}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\R}{\mathbb{R}}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{defi}{Definition}
\renewcommand{\algorithmiccomment}[1]{\% #1}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\ips}{\textnormal{IPS}}
\newcommand{\dr}{\textnormal{DR}}
\newcommand{\reg}{\textnormal{Reg}}


==> backups/ours_jr.tex <==
\begin{figure}[htb]
\vspace{1mm}
\centering
%\includegraphics[width=0.45\textwidth]{figures/completeness.png}
\includegraphics[scale=0.35]{figures/completeness.png}
%\vspace{-2mm}
\caption{\small \jihye{caption}}
\vspace{-5mm}
\label{fig:detection-completeness}
\end{figure}

\section{Proposed Method}
% \subsection{Evaluation metrics}
Given a trained DNN classifier $\bff$ and a trained OOD detector $\calD_\gamma$, our goal is to learn a set of concepts that can provide explanations for the predictions of the classifier and detector.
To this end, we first propose new metrics for quantifying a set of learned concepts, followed by a general framework for learning a set of concepts.

\subsection{Classifier and Detector in the Concept World}
\jihye{Classifier and Detector in Two Worlds}
\jihye{itemize and define world 0: , world 1}
For an input $\bfx$, consider the feature representation $\bfphi(\bfx)$, the output at a specific layer of the DNN classifier.
Without loss of generality, we focus on a convolutional layer with $\,\bfphi(\bfx) \in \reals^{a \times b \times d}$, where $d$ is the number of channels (\eg $d = 2048$), $a$ and $b$ are the filter size (\eg $a = b = 5$). Let $\bfc_i \in \reals^d, ~i = 1, \cdots, m$ denote the set of concept vectors (typically $m \ll d$).
The concept score corresponding to concept $i$ is the inner-product between the feature representation and the concept vector, \ie $\bfv_{\bfc_i}(\bfx) = \langle \bfphi(\bfx), \bfc_i \rangle \in \reals^{ab}$. This inner-product is defined as the concatenation over the $a \times b$ patch of the standard inner-products (between vectors) $\,\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle \in \reals, ~\forall p, q \in [a] \times [b]$.
The vector of concept scores from all the concepts is defined simply as the concatenation of the individual concept scores, \ie $\VC(\bfx)^T = [\bfv_{\bfc_1}(\bfx)^T, \cdots, \bfv_{\bfc_m}(\bfx)^T] \in \reals^{abm}$.

We also define a dimension-reduced version of the concept score vector that takes the maximum of the inner-product over each $a \times b$ patch (instead of concatenating them) as follows: $\TVC(\bfx)^T = [\widetilde{v}_{\bfc_1}(\bfx), \cdots, \widetilde{v}_{\bfc_m}(\bfx)] \in \reals^m$, where $\widetilde{v}_{\bfc_i}(\bfx) = \max_{p, q} |\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle|$. 
As mentioned earlier, this reduction operation is done to capture the most important correlations from each patch.

Given our assumption that the concept score vector is a sufficient statistic for the prediction of both the classifier and the detector, we define a mapping $\,\bfg : \reals^{abm} \mapsto \reals^{a \times b \times d}$ that reconstructs the feature representation at layer $\ell$ from the concept score vector.
To be precise, let $\,\recphi(\bfx) = \bfg(\VC(\bfx))$ define the reconstructed feature representation.
The mapping $\bfg$ is realized using a fully-connected neural network, whose parameters are optimized as part of the concept learning. This idea is explained in Fig.~\ref{fig:detection-completeness}.

\mypara{Classifier in the concept world.}
Given the original DNN classifier $\bff = \bfh \circ \bfphi$, we define the classifier in the ``concept world'' based on the reconstructed representation as
\begin{equation}
\label{equ:classifier_concept}
\fcon(\bfx) ~:=~ \bfh(\recphi(\bfx)) ~=~ \bfh(\bfg(\VC(\bfx))).
\end{equation}

\mypara{Detector in the concept world.}
Given an OOD detector $\calD_\gamma(\bfx, \bff)$ with score function $S(\bfx, \bff)$ for the classifier $\bff = \bfh \circ \bfphi$, we define the corresponding detector and the score function in the ``concept world'' based on the reconstructed representation as
\begin{align}
\label{equ:detector_concept}
\Dcon(\bfx, \bff) \,&:=\, \calD_\gamma(\bfx, \bfh \circ \recphi) \,=\, \calD_\gamma(\bfx, \bfh \circ \bfg \circ \VC) \nonumber \\
\Scon(\bfx, \bff) \,&:=\, S(\bfx, \bfh \circ \recphi) \,=\, S(\bfx, \bfh \circ \bfg \circ \VC).
\end{align}
Given a sufficient set of concepts $\bfC$, the classifier in the concept world should be able to closely approximate the prediction performance of the original classifier.
Likewise, the detector in the concept world should be able to closely approximate the detection performance of the original detector.
In order to concretely quantify this notion, we next define a 
% completeness score for both the classifier and the detector.
completeness score for the set of concepts with respect to the classification task and the OOD detection task.


\subsection{Completeness Score for Concepts}
\label{sec:completeness_score}
Briefly mention need for/intuition behind classification completeness by \cite{yeh2019completeness}\\.\\.\\.
%
\begin{definition}
\label{def:completeness_class}
Given a trained DNN classifier $\bff = \bfh \circ \bfphi\,$ and a set of concept vectors $\bfC$, the {\em classification completeness score} with respect to an ID distribution $\Pin(\bfx, y)$ is defined as \cite{yeh2019completeness}
\begin{align}
\label{equ: completeness-classification}
    &\eta^{}_\bff(\bfC) ~:= \\ 
    &\frac{\textrm{sup}_\bfg \,\expec_{(\bfx, y) \sim \Pin} \indicator[ y = \argmax_{y'} h_{y'}(\recphi(\bfx)) ] ~-~ a_r}{\expec_{(\bfx, y) \sim \Pin} \indicator[y = \argmax_{y'} h_{y'}(\bfphi(\bfx))] ~-~ a_r} \nonumber
\end{align}
where $\recphi(\bfx) = \bfg(\bfv_{\bfC}(\bfx))$ is the feature representation reconstructed from the concept scores, and $a_r$ is the accuracy of random prediction (\ie $a_r = 1/L$ for $L$ classes).
\end{definition}
In the numerator, the maximization is over the parameters of the fully-connected neural network $\bfg$ that reconstructs the feature representation from the vector of concept scores.
The denominator of $\eta^{}_\bff(\bfC)$ is the accuracy of the classifier $\bff$, while the numerator is the maximum accuracy that can be achieved using the feature representation reconstructed from the concept-score vector.
In practice, the expectation is estimated using a held-out test dataset $\Dinte$ from the ID distribution.

% \jihye{Limitation of the above completeness for our purpose. Need for / intuition behind detection completeness. fig (\ref{fig:detection-completeness})} \\.\\.\\.\\.\\.
% \jihye{Full elaboration on the two-world game -- fig \ref{fig:detection-completeness}}

\begin{definition}
\label{def:completeness_detec}
Given a trained DNN classifier $\bff = \bfh \circ \bfphi$, a trained OOD detector with score function $S(\bfx, \bff)$, and a set of concept vectors $\bfC$, the {\em detection completeness score} with respect to ID distribution $\Pin(\bfx, y)$ and OOD distribution $\Pout(\bfx)$ is defined as
\begin{align}
\label{equ: completeness-detection}
    \eta^{}_{\bff, S}(\bfC) 
    ~:=~ \frac{\textrm{sup}_\bfg \,\textrm{AUC}(\bfh \circ \recphi) ~-~ b_r}{\textrm{AUC}(\bfh \circ \bfphi) ~-~ b_r},
\end{align}
where $\recphi(\bfx) = \bfg(\bfv_{\bfC}(\bfx))$ is the feature representation reconstructed from the concept scores, $\textrm{AUC}(\bff)$ is the area under the ROC curve of an OOD detector for $\bff$, defined as
\begin{align}
\label{equ:auroc_ideal}
\textrm{AUC}(\bff) ~:= \!\!\expec_{(\bfx, y) \sim \Pin} \expec_{\,\bfx^\prime \sim \Pout} \indicator\big[ S(\bfx, \bff) \,>\, S(\bfx^\prime, \bff) \big],
\end{align}
and $b_r = 0.5$ is the AUROC of a random detector.
\end{definition}
As with the classification completeness, the maximization in the numerator is over the parameters of the fully-connected network $\bfg$ that reconstructs the feature representation from the vector of concept scores.
In practice, $\textrm{AUC}(\bff)$ is estimated using held-out test datasets from both the ID and OOD. Given an ID test dataset $\Dinte$ and an OOD test dataset $\Doutte$, the sample estimate of $\textrm{AUC}(\bff)$ is given by
\begin{align*}
    \widehat{\textrm{AUC}}(\bff) \,=\, \frac{1}{|\Dinte|\,|\Doutte|} \!\!\mysum_{(\bfx, y) \in \Dinte} \mysum_{~\bfx^\prime \in \Doutte} \!\!\!\indicator\big[ S(\bfx, \bff) > S(\bfx^\prime, \bff) \big]. 
\end{align*}

Both the classification completeness and detection completeness scores have a range $[0, 1]$, and a value close to $1$ indicates that the set of concepts $\bfC$ are close to complete in characterizing the behavior of the classifier and/or the OOD detector.

\subsection{Concept Separability Score}
\label{sec:separability_score}
\iffalse

% \somesh{Assumptions: enforcing separability of each individual separability --> anyway leads to better separability with combined concepts}
% \somesh{First describe the problem -what we want to do. There are these possible methods..... We chose this because of what. It should never appear like magic.}
% \somesh{Some curve -- accuracy vs separability something like that}

\jihye{need for/intuition behind separablility. Full elaboration on the idea behind separability in concept space -- fig \ref{fig:detection-separability}.} Other than the completeness scores of Eq. (\ref{equ: completeness-classification}) and Eq. (\ref{equ: completeness-detection}), we also want the concept scores between ID and OOD data to be easily distinguishable. This notion is captured by the \textit{separability} metric in Eq. (\ref{equ: distinguishability}). 

\fi
An important property that we would like to impose on the set of learned concepts for the OOD detection task is that the ID data and OOD data be well separated in the dimension-reduced concept-score space.
The motivation behind this requirement is two-fold.
The first is that we would like the concept scores to be highly distinguishable between the ID and OOD data (\eg Fig.~\ref{fig:detection-separability}), in order to effectively interpret the detector's decisions.
The second is that we would like the detector in the concept world Eq. (\ref{equ:detector_concept}) to have performance close to that of the original detector, which requires that the distribution of detector scores $\Scon(\cdot)$ from ID and OOD data be well separated.
% maybe we should say requirement of high detection completeness here?
This in-turn translates to a requirement of good separability (between ID and OOD) in the projected concept-score space.

Formally, we would like the set of concept-score vectors from the ID class $\,V_{\textrm{in}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pin\}$ and set of concept-score vectors from the OOD class $\,V_{\textrm{out}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pout\}$ to be well separated.
Let $\,J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC)) \in \reals$ define a general {\it measure of separability} between the two data subsets, such that a larger value corresponds to higher separability.
We will discuss specific choices for $J_{\textrm{sep}}$ that make it possible to tractable optimize the concept separability as part of the learning objective.

Class separability metrics have been well studied in the pattern recognition literature, particularly for the two-class case~\cite{fukunaga1990separ}~\footnote{Note that the two classes correspond to ID and OOD data.}. 
Distributional divergences such as the Kullback-Leibler and Hellinger distance can be used when the probability distribution of the two classes are known, and the divergence is tractable to compute.
Non-parametric measures of class separability (\eg based on $k$-nearest neighbors) are also candidates here, but they are usually hard to optimize using gradient-based methods.
In order to obtain a closed-form expression for the class separability, it is common to make simplifying assumptions on the class-conditional density (\eg multivariate Gaussian per class).
% We next propose a binary class separability 

\mypara{Global Concept Separability.}
Motivated by Fisher's linear discriminant analysis (LDA), we explore the use of class-separability measures based on the within-class and between-class scatter matrices~\cite{murphy2012separ}.
The goal of LDA is to find a projection vector (direction) such that data from the two classes are maximally separated and form compact clusters when projected onto this vector. 
Rather than finding an optimal projection direction, we are more interested in ensuring that the concept-score vectors from the ID and OOD data have high separability.
Given the set of concept-score vectors from the ID data $V_{\textrm{in}}(\bfC)$ and OOD data $V_{\textrm{out}}(\bfC)$, consider their within-class and between-class scatter matrices defined as
\begin{align}
\label{eq:scatter_matrices}
\bfS_w ~&= \mysum_{\bfv \in V_{\textrm{in}}(\bfC)} (\bfv \,-\, \bfmu_{\textrm{in}})\,(\bfv \,-\, \bfmu_{\textrm{in}})^T \nonumber \\
&+ \mysum_{\bfv \in V_{\textrm{out}}(\bfC)} (\bfv \,-\, \bfmu_{\textrm{out}})\,(\bfv \,-\, \bfmu_{\textrm{out}})^T, \\
%
\bfS_b ~&=~ (\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})\,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T,
\end{align}
where $\bfmu_{\textrm{in}}$ and $\bfmu_{\textrm{out}}$ are the mean concept-score vectors corresponding to the ID and OOD data respectively.
We define the following separability metric between based on the generalized eigenvalue equation solved by Fisher's LDA~\cite{fukunaga1990separ, murphy2012separ}:
\begin{align}
\label{eq:separability_trace}
&J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC)) ~=~ \textrm{tr}\big[\bfS_w^{-1} \,\bfS_b\big] \nonumber \\
% &=~ \textrm{tr}\big[\bfS_w^{-1} \,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})\,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T\big] \nonumber \\
&=~ (\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T \,\bfS_w^{-1} \,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}}).
\end{align}
Maximizing the above metric is equivalent to maximizing the sum of eigenvalues of the matrix $\,\bfS_w^{-1} \,\bfS_b$, which in-turn ensures a large between-class separability and a small within-class separability for the ID and OOD concept scores.
We refer to this as a {\em global concept separability} metric because it does not analyze the separability between the ID and OOD data on a per-class level.
% it analyzes the ID and OOD data from all the $L$ classes.

\jihye{Check if the motivation for "multivariate" separability is conveyed here.}

\mypara{Connection to the Bhattacharya distance.}
We note that the separability metric in Eq. (\ref{eq:separability_trace}) is closely related to the Bhattacharya distance~\cite{bhattacharyya1943measure} for the special case when the concept scores from both ID and OOD data follow a multivariate Gaussian density. The Bhattacharya distance is a well known measure of divergence between two probability distributions, and it has the nice property of being an upper bound to the Bayes error rate in the two-class case~\cite{fukunaga1990bhatta}. For the special case when the concept scores from both ID and OOD data follow a multivariate Gaussian with a shared covariance matrix, it can be shown that the Bhattacharya distance reduces to the separability metric in Eq. (\ref{eq:separability_trace}) (ignoring scale factors). 

\iffalse

We sometimes denote $J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC))$ as $J_{\textrm{sep}}(\bfC)$ for brevity.
Assumption of unimodal distribution; when this assumption may not be appropriate in some cases. 

\fi


\mypara{Per-Class Concept Separability.}
% Conditioned on a given predicted class
So far, we have focused on the separability between the concept scores of ID and OOD data without considering the class prediction of the classifier.
However, it may be more appropriate to impose high separability between the concept scores on a per-class level. In other words, we would like the concept scores of ID and OOD data predicted by the classifier into any given class $y \in [L]$ to be well separated.
Consider the set of concept-score vectors from ID data that are predicted into class $y$: $V^{y}_{\textrm{in}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pin, ~\widehat{y}(\bfx) = y\}$. 
Likewise, define for the OOD data $\,V^{y}_{\textrm{out}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pout, ~\widehat{y}(\bfx) = y\}$. 
We can extend the definition of the separability metric for a given predicted class $y \in [L]$ as follows
\begin{align}
\label{eq:separability_trace_per_class}
&J_{\textrm{sep}}(V^{y}_{\textrm{in}}(\bfC), V^{y}_{\textrm{out}}(\bfC)) ~=~ \textrm{tr}\big[(\bfS^{y}_w)^{-1} \,\bfS^y_b\big] \nonumber \\
&=~ (\bfmu^y_{\textrm{out}} \,-\, \bfmu^y_{\textrm{in}})^T \,(\bfS^y_w)^{-1} \,(\bfmu^y_{\textrm{out}} \,-\, \bfmu^y_{\textrm{in}}).
\end{align}
The scatter matrices $\bfS^y_w$ and $\bfS^y_b$ are defined similar to Eq. (\ref{eq:scatter_matrices}), using the per-class subset of concept scores $V^{y}_{\textrm{in}}(\bfC)$ or $V^{y}_{\textrm{out}}(\bfC)$, and the mean concept-score vectors from the ID and OOD data are also defined at a per-class level.

\jayaram{Need to say something more here. About how the global and per-class separability metrics are used.}

We sometimes use the notation $J_{\textrm{sep}}(\bfC)$ instead of $J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC))$ and $J^y_{\textrm{sep}}(\bfC)$ instead of $J_{\textrm{sep}}(V^{y}_{\textrm{in}}(\bfC), V^{y}_{\textrm{out}}(\bfC))$ for brevity.

% In practice, a held-out validation dataset is used
% Define shorthand notations for the separability metrics.


\iffalse

% Separability literature (BC distance... assumptions.. special case: trace)
% \\.\\.\\.\\.\\.\\.\\.\\.

Given datasets $D_{\text{in}}^{l} = \{(\bfx_i, y_i) | y_i = l\}_{i=1}^{N_{in}^{l}}$ and $D_{\text{out}}^{l} = \{\bfx_i | y_i = l\}_{i=1}^{N_{out}^{l}}$, for each concept $k = 1, 2, ..., m$ and class label $l = 1, 2, ..., L$.
\begin{enumerate}
\item First, we compute means of concept scores for each concept: for ID cluster, $\mu_{in}^{l, k} = \frac{1}{N_{in}^l}\sum_{\bfx_i \in D^{l}_{in}} v_{\bfc_k}(\bfx_i)$ and for OOD cluster, $\mu_{out}^{l, k} = \frac{1}{N_{out}^l}\sum_{\bfx_i \in D^{l}_{out}} v_{\bfc_k}(\bfx_i)$ where $v_{\bfc_k}(\bfx_i)$ is the score with respect to the $k$-th concept $\bfc_k$.
We desire $\mu_{in}^{l, k}$ and $\mu_{out}^{l, k}$ to be as far as possible to each other.
\item Second, we compute intra-cluster scatters for each concept: for ID cluster, $s_{in}^{l, k} = \sum_{\bfx_i \in D^{l}_{in}} (v_{\bfc_k}(\bfx_i) - \mu_{in}^k)^2$ and for OOD cluster, $s_{out}^k = \sum_{\bfx_i \in D^{l}_{out}} (v_{\bfc_k}(\bfx_i) - \mu_{out}^k)^2$.
We desire $s_{in}^{l,k}$ and $s_{out}^{l,k}$ to be as small as possible.
\item Then the separability between the ID cluster and OOD cluster is measured as follows,
\begin{equation*}
    J^l(\bfc_k) = \frac{(\mu_{in}^k - \mu_{out}^k)^2}{(s_{in}^k + s_{out}^k)}
\end{equation*}
\begin{equation}
\label{equ: separability}
    J(\bfC) = \frac{1}{L \cdot m}\sum_{l=1}^L\sum_{k=1}^m J^l(\bfc_k)
\end{equation}
Higher score for $J(\bfC)$ indicates the better distinguishability between ID concept scores and OOD concept scores.
\end{enumerate}

Note the close relation to Fisher Linear Discriminant (FLD). FLD finds the optimal projection from high resolution input data into low dimensional representations that maximizes the separability between classes.
Let $\{\bfphi_1, \bfphi_2, .., \bfphi_n\}$ be $d$-dimensional samples that belong to one of binary classes, $y_i = \{0, 1\}$. \jihye{notation for detection vs notation for classification -- clarify!}
$\bfphi_i$ is the feature representation at layer $l$ flattened into $d$-dimensional vector: $\bfphi_i = \phi(\bfx_i)$.
Let $\bfv$ be a unit vector in the $d$-dimensional space and $z_i = \bfv\cdot\bfphi_i$ is the projection of $\bfphi_i$ into a one dimensional subspace.
Let $\mu_0 = \frac{1}{n_0}\sum_{z_i: y_i = 0}^{n_0} z_i = \bfv \cdot (\frac{1}{n_0}\sum_{\bfphi_i: y_i = 0}^{n_0} \bfphi_i)$ be the mean of projected values for class 0 and similarly, $\mu_1$ be the mean for class 1.
Define scatter for class 0 as $s_0 = \sum_{z_i: y_i = 0}^{n_0} (z_i - \mu_0)^2$ and similarly, $s_1$ is the scatter for class 1.
$s_0$ can be rewritten in a vector form as,
\begin{align*}
    s_0 &= \sum_{z_i: y_i = 0}^{n_0} (z_i - \mu_0)^2 = \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfv \cdot (\bfphi_i - \bfmu_0))^2 \\
    &= \bfv^\mathsf{T} \cdot \left \Big[ \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfphi_i - \bfmu_0) \cdot (\bfphi_i - \bfmu_0)^\mathsf{T} \right \Big] \cdot \bfv
\end{align*}
where $\bfmu_0 = \frac{1}{n_0}\sum_{\bfphi_i: y_i = 0}^{n_0} \bfphi_i$ is the sample mean for class 0.
Let $S_w$ be the within class scatter matrix: $S_w = \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfphi_i - \bfmu_0) \cdot (\bfphi_i - \bfmu_0)^\mathsf{T} + \sum_{\bfphi_i: y_i = 1}^{n_1} (\bfphi_i - \bfmu_1) \cdot (\bfphi_i - \bfmu_1)^\mathsf{T}$. Then FLD measures the separability with respect to $\bfv$ as, 
\begin{equation}
    \label{equ: FLD}
    J_{Fisher}(\bfv) = \frac{(\mu_0 - \mu_1)^2}{(s_0 + s_1)} = \frac{\bfv^\mathsf{T} \cdot (\bfmu_0 - \bfmu_1)(\bfmu_0 - \bfmu_1)^\mathsf{T} \cdot \bfv }{\bfv^\mathsf{T} \cdot S_w \cdot \bfv}
\end{equation}
FLD finds $\widetilde{\bfv}$ such that $\frac{d J(\widetilde{\bfv})}{d \bfv} = 0$ for the optimal projection with maximum separability: $\widetilde{\bfv} = S_w^{-1}(\bfmu_0 - \bfmu_1)$.

Finally, our distinguishability index given a set of concept vectors $\bfC = \{\bfc_1, \bfc_2, ..., \bfc_m\}$ is defined as,
\begin{equation}
    \label{equ: distinguishability}
    S(\bfC) = \frac{J(\bfC)}{J_{Fisher}(\widetilde{\bfv})}
\end{equation}
% Guan et al. introduces Distance-based Separability Index (DSI) that measures how the distribution of intra-class distance (ICD) resembles the distribution of between-class distance (BCD) through statistical testing ~\cite{separability}. As the two classes are more separable, ICD and BCD are more distinguishable. 
% They verify the DSI to be more effective in measuring the separability of both synthetic and real-world datasets, compared to other separability indices such as Fisher discriminant ratio, neighborhood measures and linearity measures.
% We adopt DSI to quantify how distinguishable the ID concept scores and OOD concept scores are.
% Given $D_{\text{in}}^{test} = \{(\bfx_i, y_i)\}_{i=1}^{N_{in}}$ and $D_{\text{out}}^{test} = \{\bfx_i\}_{i=1}^{N_{out}}$, and a set of concept vectors $\bfC = \{\bfc\}_i^m$, we compute separability score between ID and OOD:
% \begin{enumerate}
%     \item First, we prepare $S_{in} = \{s_1, s_2, ..., s_{N_{in}}~|~s_i = v_\bfC(\bfx_i), \bfx_i \in D^{test}_{in}\}$ and $S_{out} = \{s_1, s_2, ..., s_{N_{out}}~|~s_i = v_\bfC(\bfx_i), \bfx_i \in D^{test}_{out}\}$. These are the set of concept scores for ID and OOD data, respectively.
    
%     \item ICD set for ID data, $\{d_{in}\}$ is a set of $l_2$ distances between any two points in $S(D_{\text{in}}^{test})$: $\{d_{in}\} = \{||s_i - s_j||_2 ~|~ s_i, s_j \in S_{in}; s_i \neq s_j\}$.
%     Likewise, $\{d_{out}\}$ is the ICD set for OOD data.
    
%     \item BCD set between ID and OOD data, $\{d_{in, out}\}$ is the set of $l_2$ distances between any two points from different distribution (ID and OOD): $\{d_{in, out}\} = \{||s_{in} - s_{out}||_2 ~|~ s_{in} \in S_{in}, s_out \in S_{out}\}$.
    
%     \item Then, the similarity between the ICD and BCD sets are computed using the Kolmogorov-Smirnov (KS) distance:
%     \[k_{in} = KS(\{d_{in}\}, \{d_{in, out}\}), \textrm{and}~ k_{out} = KS(\{d_{out}\}, \{d_{in, out}\})\]
%     \item Finally, the DSI of ID and OOD data is computed by averaging the two KS distances as follows,
%     \begin{equation}
%         \label{equ: separability}
%         DSI(D_{\text{in}}^{test}, D_{\text{out}}^{test}) = \frac{(k_{in} + k_{out})}{2}
%     \end{equation}
% \end{enumerate}

\fi


\subsection{Proposed Concept Learning Algorithm}
\label{sec:concept_learning}

\label{alg:concept_learning}
\begin{algorithm}
\caption{Learning concepts for OOD detector}
\begin{algorithmic}[1]
  \INPUT: Entire training set $\Dtr = \{\Dintr, \Douttr\}$, entire validation set $\Dval = \{\Dinval, \Doutval\}$, classifier $\bff$, detector $\calD$;
  \OUTPUT: $\bfC$, $g$
  \STATE initialize $\bfC$ and parameters of $g$;
  \STATE identify threshold $\gamma$ for $\calD_\gamma(\bfx, \bff)$ on $\Dval$, and prepare $\widehat{\Dinval}$ and $\widehat{\Doutval}$;
  \FOR{$i = 0, 1, 2, ... $}
    \STATE 
    \STATE 
	\STATE 
    \STATE Update $g$ and $\bfC$ using Eqn. \ref{equ: concept learning}: \\
	\quad Option I: 
  \ENDFOR
%   \RETURN $g$
\end{algorithmic}
\end{algorithm}

In this section, we develop our proposed concept learning objective that aims to find a set of concepts $\bfC = \{\bfc_1, \bfc_2, ..., \bfc_m\}$ and a mapping $\bfg$ (parameterized by a neural network) that have the following properties: 1) high detection completeness w.r.t the given OOD detector; 2) high classification completeness w.r.t the DNN classifier; and 3) high separability in the concept-score space between the samples detected as ID and the samples detected as OOD by the detector. 

\mypara{Limitation of Previous Work.} 
\cite{yeh2019completeness} 
The baseline concept learning objective by \cite{yeh2019completeness} aims to find a set of concepts $\bfC$ and a mapping $\bfg$ (parameterized by a neural network) that jointly maximize the recovered accuracy of the classifier in the concept world.
% to maximize the completeness of the learned concepts $\bfC = \{\bfc_1, \bfc_2, ..., \bfc_m\}$ for the classification task as follows,
\begin{equation}
\label{equ: baseline}
    \argmax_{\bfC, \bfg} \expec_{(\bfx, y) \sim \Pin}\!\!\big[ \log h_y(\bfg(\VC(\bfx))) \big] ~+~ \lambda_{\textrm{expl}}\, R_{\textrm{expl}}(\bfC),
\end{equation}
where $R_{\textrm{expl}}(\bfC)$ is a regularization term used to ensure that the learned concept vectors have high spatial coherancy and low redundancy (among themselves). It is defined as
\begin{align}
\label{equ:regularizer_expl}
    R_{\textrm{expl}}(\bfC) ~&=~ \frac{1}{m\,K} \mysum_{k=1}^m \mysum_{\bfx^\prime \in T_{\bfc_k}} \langle \bfphi(\bfx^\prime), \bfc_k \rangle \nonumber \\
    &-~ \frac{1}{m \,(m - 1)} \mysum_{j=1}^m \mysum_{k=j + 1}^m \langle \bfc_j, \bfc_k \rangle.
\end{align}
Here $T_{\bfc_k}$ is the set of $K$-nearest neighbor patches of the concept vector $\bfc_k$ from the ID training set $\Dintr$.
 


Unfortunately, the objective in Eq. (\ref{equ: baseline}) does not guarantee that the recovered feature representation $\recphi(\bfx)$ would match the original feature representation $\bfphi(\bfx)$.
Even when the recovered accuracy matches the original classification accuracy, if $\recphi(\bfx)$ and $\bfphi(\bfx)$ are not sufficiently close, the representations at the penultimate layer would vary a lot, leading to unmatched detection results by $\mathcal{D}$.
Hence, we include an additional regularization term that minimizes the $\ell_2$ distance 
% \begin{equation}
% \label{equ: baseline+l2}
%     \argmax_{\bfC, g} \, \text{log} \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] + \lambda_1 \cdot R_{coherency}(\bfC) + \lambda_2 \cdot
%     \expec_{\bfx \sim D_{train}^{in}}||\phi(\bfx) - \hat{\phi}_{g, \bfC}(\bfx))||_2
% \end{equation}
% \begin{equation}
% \label{equ: baseline+score}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) ~-~ \alpha \expec_{\bfx \sim D_{train}^{in}} (\mathcal{D}(h(\hat{\phi}_{g, \bfC}(\bfx))) - \mathcal{D}(f(\bfx)))^2
% \end{equation}

% Let $D^{train} = \{D_{\text{in}}^{train} \cup D_{\text{out}}^{train}\}$, and data is drawn as $(\bfx, s) \sim D^{train}$ where $s \in \{0, 1\}$ is the groundtruth label of OOD detection.
%
% \begin{equation}
% \label{equ: baseline+separability}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) ~+~ \beta \expec_{\bfx \sim D^{train}} J(\bfC)
% \end{equation}
%

\begin{align}
\label{equ: concept learning}
\argmax_{\bfC, g}\, &\log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda_{\textrm{expl}}\, R_{\textrm{expl}}(\bfC) \nonumber \\
&-~ \lambda_{\textrm{mse}}\, \expec_{\bfx \sim \Dtr} (\Dcon(\bfx, \bff) - \calD_\gamma(\bfx, \bff))^2 \nonumber \\
&-~ \lambda_{\textrm{norm}}\, \expec_{\bfx \sim \Dintr}||\bfphi(\bfx) - \recphi(\bfx)||^2 \nonumber \\
&+~ \lambda_{\textrm{sep}}~J(\bfC)
\end{align}
\jihye{shall we need some algorithm block?}
%
% Note that using \begin{align} ... \end{align} is a better way that using \begin{array}
% \begin{equation}
% \label{equ: concept learning}
% \begin{array}{l}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) \hspace{20mm} \\
%     -~ \alpha\, \expec_{\bfx \sim D^{train}}\mathcal{D}(h(\hat{\phi}_{g, \bfC}(\bfx))) - \mathcal{D}(f(\bfx)))^2 
%     ~+~ \beta\, \expec_{\bfx \sim D^{train}} J(\bfC) \\
%     -~ \gamma\, \expec_{\bfx \sim D^{train}}||\phi(\bfx) - \hat{\phi}_{g, \bfC}(\bfx))||_2
% \end{array}
% \end{equation}



==> backups/ours_old.tex <==
\section{Proposed Method}
Given a trained DNN classifier $\bff$ and a paired OOD detector $\calD_\gamma$, our goal is to learn a set of concepts that can provide explanations for the predictions of the detector.
We first propose new metrics for quantifying the set of learned concepts, followed by a general framework for learning the concepts.
% This section explains our evaluation metrics and methods: (1) how to gauge the utility of a given set of concepts for OOD detector explanation, and (2) a general learning algorithm to discover concepts that \jihye{incomplete yet}

\mypara{ID and OOD Datasets.}
% Throughout the paper, 
We assume the availability of a labeled ID training dataset $\Dintr = \{(\bfx_i, y_i), ~i = 1, \cdots, \Nintr\}$ from the distribution $\Pin$, where $y_i \in \outputs$ is the class label for an input $\bfx_i \in \inputs$.
We also assume the availability of an unlabeled training dataset $\Douttr = \{\widetilde{\bfx}_i, ~i = 1, \cdots,  \Nouttr\}$ from a different distribution, referred to as the {\em auxiliary OOD dataset}.
Similarly, we define the ID validation and test datasets (sampled from $\Pin$) as $\Dinval$ and $\Dinte$, and the OOD validation and test datasets as $\Doutval$ and $\Doutte$.
We note that the auxiliary OOD dataset $\Dintr$ and validation OOD dataset $\Dinval$ are sampled from the same auxiliary distribution (\eg the MS-COCO dataset). However, the test OOD dataset can be from an entirely different and unknown distribution (\eg the SUN dataset), as is often the case in reality.
% Add notation for the number of samples if needed.
All the OOD datasets are unlabeled since their label space can be different from $\outputs$. One can think of the OOD datasets for training, validation, and test to be biased samples from an unknown OOD marginal distribution $\Pout(\bfx)$.

\mypara{Concept Scores.}
We start by formalizing how to compute a representative score for concepts given an input, which will be used for evaluation in Section \ref{sec:completeness_score} and Section \ref{sec:separability_score}.
A projection matrix $\bfC \in \reals^{d_\ell \times m}$ that maps $\bfphi(\bfx)$ to $\bfv_{\bfC}(\bfx)$ consists of $m$ unit (column) vectors $\,\bfC := [\bfc_1 \cdots \bfc_m]$, where each $\bfc_i$ is referred to as a \textit{concept vector} representing the $i$-th concept (\eg "stripe", "oval face", etc.), and $m$ is the number of concepts.
The inner product between the feature representation and a concept vector quantifies how close the input is to the given concept, and this is referred to as the concept score. 
Specifically, the concept score correicsponding to concept $i$ is $\bfv_{\bfc_i}(\bfx) = \langle \bfphi(\bfx), \bfc_i \rangle \in \reals^{a_\ell b_\ell}$, which is the $a_\ell \times b_\ell$ times concatenation over the standard inner-products (between vectors) $\,\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle \in \reals, ~\forall p, q \in [a_\ell] \times [b_\ell]$, where $\bfphi^{p,q}$ is the feature representation corresponding to the $(p, q)$-th patch of input $\bfx$ (\ie receptive field).
That is, $\bfv_{\bfc_i}(\bfx)$ \ryan{maybe $\bfv_{\bfc_i}^{(p,q)}(\bfx)?$} is the concept score of $(p, q)$-th patch of $\bfx$ with respect to $i$-th concept, and if it is a large positive (or negative) value, then the corresponding part of input is positively (or negatively) aligned with the concept.
The vector of concept scores from all the concepts is defined simply as the concatenation of the individual concept scores, \ie $\VC(\bfx)^T = [\bfv_{\bfc_1}(\bfx)^T, \cdots, \bfv_{\bfc_m}(\bfx)^T] \in \reals^{a_\ell b_\ell m}$.

% When $p = q = 1$ for fully-connected layers (\ie the receptive field of $\bfphi$ corresponds to the entire input $\bfx_i$), $\langle \bfphi(\bfx_i),~\bfc_j \rangle$ is a scalar concept score that represents the input.
% On the other hand, when $p, q > 1$, to obtain a scalar concept score for a given input, we take the maximum absolute concept score across the $p \times q$ patches, corresponding to $p \times q$ feature representations.
% To define the overall closeness of an input $\bfx_i$ and the concept $\bfc_j$ with a scalar concept score, we take the maximum absolute concept score across the $p \times q$ patches of $\bfx_i$.
When $p, q > 1$ (unless a fully-connected layer is of interest), where the receptive field of $\bfphi$ corresponds to the entire input $\bfx_i$), we also define a dimension-reduced version of the concept score vector that takes the maximum of the inner-product over each $a_\ell \times b_\ell$ patch (instead of concatenating them) as follows: $\TVC(\bfx)^T = [\widetilde{v}_{\bfc_1}(\bfx), \cdots, \widetilde{v}_{\bfc_m}(\bfx)] \in \reals^m$, where $\widetilde{v}_{\bfc_i}(\bfx) = \max_{p, q} |\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle| \in \reals$.
% The intuition behind taking a maximum score across the patches of input is as follows.
This reduction operation is done to capture the most important correlations from each patch.
Suppose $\bfc_j$ represents a striped pattern and $\bfx_i$ is an image of a zebra standing on grass.
The patch of greenery background should get a low concept score, while a patch of the zebra's body should get high concept score.
% As the defining score for the stripe concept, we decide to take the score from the patch of zebra's body, out of all patches constituting the entire input image.
Out of all the patches constituting the input image, we take the maximum score (likely) corresponding to a patch of the zebra's body as the defining score for the striped concept.

Based on the concept scores and data defined as above, we elaborate the evaluation criteria of concepts for the purpose of OOD detector explanation in Section \ref{sec:completeness_score} and Section \ref{sec:separability_score}, followed by a general learning algorithm to discover concepts that satisfy the criteria in Section \ref{sec:concept_learning}.

\subsection{Completeness Score for Concepts}
\label{sec:completeness_score}
In this subsection, we address the following questions \ryan{: 1) are the set of learned concepts $\bfC$ sufficient to similarly match the behavior of the original classifier $\bff$ and 2) are the set of learned concepts $\bfC$ sufficient to similarly match the behavior of the OOD detector $\calD$? Such properties would indicate that the concepts learned are appropriate for describing the behavior of $\bfC$ and $\calD$. }: \textit{}
\jihye{yes, I'm still working on this paragraph}

% Given a trained DNN classifier $\bff$ and a trained OOD detector $\calD_\gamma$, our goal is to learn a set of concepts that can provide explanations for the predictions of the classifier and detector.
% To this end, we first propose new metrics for quantifying a set of learned concepts, followed by a general framework for learning a set of concepts.


Given a sufficient set of concepts $\bfC$, the classifier in the concept world should be able to closely approximate the prediction performance of the original classifier.
Likewise, the detector in the concept world should be able to closely approximate the detection performance of the original detector.
In order to concretely quantify this notion, we next define a 
completeness score for the set of concepts with respect to the classification task and the OOD detection task.

\begin{definition}
\label{def:completeness_class}
Given a trained DNN classifier $\bff = \bfh \circ \bfphi\,$ and a set of concept vectors $\bfC$, the {\em classification completeness score} with respect to an ID distribution $\Pin(\bfx, y)$ is defined as in \cite{yeh2019completeness}:
\begin{align}
\label{equ: completeness-classification}
    &\eta^{}_\bff(\bfC) ~:= \\ 
    &\frac{\textrm{sup}_\bfg \,\expec_{(\bfx, y) \sim \Pin} \indicator[ y = \argmax_{y'} h_{y'}(\recphi(\bfx)) ] ~-~ a_r}{\expec_{(\bfx, y) \sim \Pin} \indicator[y = \argmax_{y'} h_{y'}(\bfphi(\bfx))] ~-~ a_r} \nonumber
\end{align}
where $a_r$ is the accuracy of random prediction (\ie $a_r = 1/L$ for $L$ classes).
\end{definition}
In the numerator, the maximization is over the parameters of the fully-connected neural network $\bfg$ that reconstructs the feature representation from the vector of concept scores \jihye{is this sentence necessary?}.
The denominator of $\eta^{}_\bff(\bfC)$ is the accuracy of the classifier $\bff$ in canonical world, while the numerator is the maximum accuracy that can be achieved using the feature representation reconstructed from the concept-score vector in concept world.
In practice, the expectation is estimated using a held-out test dataset $\Dinte$ from the ID distribution.

% \jihye{Limitation of the above completeness for our purpose. Need for / intuition behind detection completeness. fig (\ref{fig:detection-completeness})} \\.\\.\\.\\.\\.
% \jihye{Full elaboration on the two-world game -- fig \ref{fig:detection-completeness}}

\begin{definition}
\label{def:completeness_detec}
Given a trained DNN classifier $\bff = \bfh \circ \bfphi$, a trained OOD detector with score function $S(\bfx, \bff)$, and a set of concept vectors $\bfC$, the {\em detection completeness score} with respect to ID distribution $\Pin(\bfx, y)$ and OOD distribution $\Pout(\bfx)$ is defined as
\begin{align}
\label{equ: completeness-detection}
    \eta^{}_{\bff, S}(\bfC) 
    ~:=~ \frac{\textrm{sup}_\bfg \,\textrm{AUC}(\bfh \circ \recphi) ~-~ b_r}{\textrm{AUC}(\bfh \circ \bfphi) ~-~ b_r},
\end{align}
% where $\recphi(\bfx) = \bfg(\bfv_{\bfC}(\bfx))$ is the feature representation reconstructed from the concept scores, 
where $\textrm{AUC}(\bff)$ is the area under the ROC curve of an OOD detector for $\bff$, defined as
\begin{align}
\label{equ:auroc_ideal}
\textrm{AUC}(\bff) ~:= \!\!\expec_{(\bfx, y) \sim \Pin} \expec_{\,\bfx^\prime \sim \Pout} \indicator\big[ S(\bfx, \bff) \,>\, S(\bfx^\prime, \bff) \big],
\end{align}
and $b_r = 0.5$ is the AUROC of a random detector.
\end{definition}
As with the classification completeness, the maximization in the numerator is over the parameters of the fully-connected network $\bfg$ that reconstructs the feature representation from the vector of concept scores \jihye{is this sentence necessary?}.
In practice, $\textrm{AUC}(\bff)$ is estimated using held-out test datasets from both the ID and OOD. Given an ID test dataset $\Dinte$ and an OOD test dataset $\Doutte$, the sample estimate of $\textrm{AUC}(\bff)$ is given by
\begin{align*}
    \widehat{\textrm{AUC}}(\bff) \,=\, \frac{1}{|\Dinte|\,|\Doutte|} \!\!\mysum_{(\bfx, y) \in \Dinte} \mysum_{~\bfx^\prime \in \Doutte} \!\!\!\indicator\big[ S(\bfx, \bff) > S(\bfx^\prime, \bff) \big]. 
\end{align*}

Both the classification completeness and detection completeness scores have a range $[0, 1]$ \jihye{technically, $> 1$ is possible} \ryan{probably worth explaining how this can happen}, and a value close to $1$ indicates that the set of concepts $\bfC$ are close to complete in characterizing the behavior of the classifier and/or the OOD detector.

\subsection{Concept Separability Score}
\label{sec:separability_score}
\iffalse

% \somesh{Assumptions: enforcing separability of each individual separability --> anyway leads to better separability with combined concepts}
% \somesh{First describe the problem -what we want to do. There are these possible methods..... We chose this because of what. It should never appear like magic.}
% \somesh{Some curve -- accuracy vs separability something like that}

\jihye{need for/intuition behind separablility. Full elaboration on the idea behind separability in concept space -- fig \ref{fig:detection-separability}.} Other than the completeness scores of Eq. (\ref{equ: completeness-classification}) and Eq. (\ref{equ: completeness-detection}), we also want the concept scores between ID and OOD data to be easily distinguishable. This notion is captured by the \textit{separability} metric in Eq. (\ref{equ: distinguishability}). 


An important property that we would like to impose on the set of learned concepts for the OOD detection task is that the ID data and OOD data be well separated in the dimension-reduced concept-score space.
The motivation behind this requirement is two-fold.
The first is that we would like the concept scores to be highly distinguishable between the ID and OOD data (\eg Fig.~\ref{fig:detection-separability}), in order to effectively interpret the detector's decisions.
The second is that we would like the detector in the concept world Eq. (\ref{equ:detector_concept}) to have performance close to that of the original detector, which requires that the distribution of detector scores $\Scon(\cdot)$ from ID and OOD data be well separated.
% maybe we should say requirement of high detection completeness here?
This in-turn translates to a requirement of good separability (between ID and OOD) in the projected concept-score space.
\fi

;Formally, we would like the set of concept-score vectors from the ID class $\,V_{\textrm{in}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pin\}$ and set of concept-score vectors from the OOD class $\,V_{\textrm{out}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pout\}$ to be well separated \ryan{to help ensure clear distinctions in the explanations between ID and OOD}.
Let $\,J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC)) \in \reals$ define a general {\it measure of separability} between the two data subsets, such that a larger value corresponds to higher separability.
We will discuss specific choices for $J_{\textrm{sep}}$ that make it possible to tractable optimize the concept separability as part of the learning objective.

Class separability metrics have been well studied in the pattern recognition literature, particularly for the two-class case~\cite{fukunaga1990separ}~\footnote{Note that the two classes correspond to ID and OOD data.}. 
Distributional divergences such as the Kullback-Leibler and Hellinger distance can be used when the probability distribution of the two classes are known, and the divergence is tractable to compute.
Non-parametric measures of class separability (\eg based on $k$-nearest neighbors) are also candidates here, but they are usually hard to optimize using gradient-based methods.
In order to obtain a closed-form expression for the class separability, it is common to make simplifying assumptions on the class-conditional density (\eg multivariate Gaussian per class).
% We next propose a binary class separability 

\mypara{Global Concept Separability.}
Motivated by Fisher's linear discriminant analysis (LDA), we explore the use of class-separability measures based on the within-class and between-class scatter matrices~\cite{murphy2012separ}.
The goal of LDA is to find a projection vector (direction) such that data from the two classes are maximally separated and form compact clusters when projected onto this vector. 
Rather than finding an optimal projection direction, we are more interested in ensuring that the concept-score vectors from the ID and OOD data have high separability.
Given the set of concept-score vectors from the ID data $V_{\textrm{in}}(\bfC)$ and OOD data $V_{\textrm{out}}(\bfC)$, consider their within-class and between-class scatter matrices defined as
\begin{align}
\label{eq:scatter_matrices}
\bfS_w ~&= \mysum_{\bfv \in V_{\textrm{in}}(\bfC)} (\bfv \,-\, \bfmu_{\textrm{in}})\,(\bfv \,-\, \bfmu_{\textrm{in}})^T \nonumber \\
&+ \mysum_{\bfv \in V_{\textrm{out}}(\bfC)} (\bfv \,-\, \bfmu_{\textrm{out}})\,(\bfv \,-\, \bfmu_{\textrm{out}})^T, \\
%
\bfS_b ~&=~ (\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})\,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T,
\end{align}
where $\bfmu_{\textrm{in}}$ and $\bfmu_{\textrm{out}}$ are the mean concept-score vectors corresponding to the ID and OOD data respectively.
We define the following separability metric between based on the generalized eigenvalue equation solved by Fisher's LDA~\cite{fukunaga1990separ, murphy2012separ}:
\begin{align}
\label{eq:separability_trace}
&J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC)) ~=~ \textrm{tr}\big[\bfS_w^{-1} \,\bfS_b\big] \nonumber \\
% &=~ \textrm{tr}\big[\bfS_w^{-1} \,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})\,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T\big] \nonumber \\
&=~ (\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}})^T \,\bfS_w^{-1} \,(\bfmu_{\textrm{out}} \,-\, \bfmu_{\textrm{in}}).
\end{align}
Maximizing the above metric is equivalent to maximizing the sum of eigenvalues of the matrix $\,\bfS_w^{-1} \,\bfS_b$, which in-turn ensures a large between-class separability and a small within-class separability for the ID and OOD concept scores.
We refer to this as a {\em global concept separability} metric because it does not analyze the separability between the ID and OOD data on a per-class level.
% it analyzes the ID and OOD data from all the $L$ classes.

\jihye{Check if the motivation for "multivariate" separability is conveyed here.}

\mypara{Connection to the Bhattacharya distance.}
We note that the separability metric in Eq. (\ref{eq:separability_trace}) is closely related to the Bhattacharya distance~\cite{bhattacharyya1943measure} for the special case when the concept scores from both ID and OOD data follow a multivariate Gaussian density. The Bhattacharya distance is a well known measure of divergence between two probability distributions, and it has the nice property of being an upper bound to the Bayes error rate in the two-class case~\cite{fukunaga1990bhatta}. For the special case when the concept scores from both ID and OOD data follow a multivariate Gaussian with a shared covariance matrix, it can be shown that the Bhattacharya distance reduces to the separability metric in Eq. (\ref{eq:separability_trace}) (ignoring scale factors). 

\iffalse

We sometimes denote $J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC))$ as $J_{\textrm{sep}}(\bfC)$ for brevity.
Assumption of unimodal distribution; when this assumption may not be appropriate in some cases. 

\fi


\mypara{Per-Class Concept Separability.}
% Conditioned on a given predicted class
So far, we have focused on the separability between the concept scores of ID and OOD data without considering the class prediction of the classifier.
However, it may be more appropriate to impose high separability between the concept scores on a per-class level. In other words, we would like the concept scores of ID and OOD data predicted by the classifier into any given class $y \in [L]$ to be well separated.
Consider the set of concept-score vectors from ID data that are predicted into class $y$: $V^{y}_{\textrm{in}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pin, ~\widehat{y}(\bfx) = y\}$. 
Likewise, define for the OOD data $\,V^{y}_{\textrm{out}}(\bfC) := \{\TVC(\bfx) \in \reals^m ~:~ \bfx \sim \Pout, ~\widehat{y}(\bfx) = y\}$. 
We can extend the definition of the separability metric for a given predicted class $y \in [L]$ as follows
\begin{align}
\label{eq:separability_trace_per_class}
&J_{\textrm{sep}}(V^{y}_{\textrm{in}}(\bfC), V^{y}_{\textrm{out}}(\bfC)) ~=~ \textrm{tr}\big[(\bfS^{y}_w)^{-1} \,\bfS^y_b\big] \nonumber \\
&=~ (\bfmu^y_{\textrm{out}} \,-\, \bfmu^y_{\textrm{in}})^T \,(\bfS^y_w)^{-1} \,(\bfmu^y_{\textrm{out}} \,-\, \bfmu^y_{\textrm{in}}).
\end{align}
The scatter matrices $\bfS^y_w$ and $\bfS^y_b$ are defined similar to Eq. (\ref{eq:scatter_matrices}), using the per-class subset of concept scores $V^{y}_{\textrm{in}}(\bfC)$ or $V^{y}_{\textrm{out}}(\bfC)$, and the mean concept-score vectors from the ID and OOD data are also defined at a per-class level.


\ryan{Ideally, high global concept separability would ensure on a macro level that the concepts provide clear explanations regardless of the class and decision of the classifier. But, as the goal is to provide concept explanations for OOD detectors, we could still provide meaningful explanations on a per-class basis if we can separate out concepts that are from an OOD image classified as a certain class $c$ versus and ID image classified as $c$. Examining both metrics help us gauge the relative separability on finer and coarser scales to evaluate the quality of the concept explanations.}
\jayaram{Need to say something more here. About how the global and per-class separability metrics are used.}

We sometimes use the notation $J_{\textrm{sep}}(\bfC)$ instead of $J_{\textrm{sep}}(V_{\textrm{in}}(\bfC), V_{\textrm{out}}(\bfC))$ and $J^y_{\textrm{sep}}(\bfC)$ instead of $J_{\textrm{sep}}(V^{y}_{\textrm{in}}(\bfC), V^{y}_{\textrm{out}}(\bfC))$ for brevity.

% In practice, a held-out validation dataset is used
% Define shorthand notations for the separability metrics.


\iffalse

% Separability literature (BC distance... assumptions.. special case: trace)
% \\.\\.\\.\\.\\.\\.\\.\\.

Given datasets $D_{\text{in}}^{l} = \{(\bfx_i, y_i) | y_i = l\}_{i=1}^{N_{in}^{l}}$ and $D_{\text{out}}^{l} = \{\bfx_i | y_i = l\}_{i=1}^{N_{out}^{l}}$, for each concept $k = 1, 2, ..., m$ and class label $l = 1, 2, ..., L$.
\begin{enumerate}
\item First, we compute means of concept scores for each concept: for ID cluster, $\mu_{in}^{l, k} = \frac{1}{N_{in}^l}\sum_{\bfx_i \in D^{l}_{in}} v_{\bfc_k}(\bfx_i)$ and for OOD cluster, $\mu_{out}^{l, k} = \frac{1}{N_{out}^l}\sum_{\bfx_i \in D^{l}_{out}} v_{\bfc_k}(\bfx_i)$ where $v_{\bfc_k}(\bfx_i)$ is the score with respect to the $k$-th concept $\bfc_k$.
We desire $\mu_{in}^{l, k}$ and $\mu_{out}^{l, k}$ to be as far as possible to each other.
\item Second, we compute intra-cluster scatters for each concept: for ID cluster, $s_{in}^{l, k} = \sum_{\bfx_i \in D^{l}_{in}} (v_{\bfc_k}(\bfx_i) - \mu_{in}^k)^2$ and for OOD cluster, $s_{out}^k = \sum_{\bfx_i \in D^{l}_{out}} (v_{\bfc_k}(\bfx_i) - \mu_{out}^k)^2$.
We desire $s_{in}^{l,k}$ and $s_{out}^{l,k}$ to be as small as possible.
\item Then the separability between the ID cluster and OOD cluster is measured as follows,
\begin{equation*}
    J^l(\bfc_k) = \frac{(\mu_{in}^k - \mu_{out}^k)^2}{(s_{in}^k + s_{out}^k)}
\end{equation*}
\begin{equation}
\label{equ: separability}
    J(\bfC) = \frac{1}{L \cdot m}\sum_{l=1}^L\sum_{k=1}^m J^l(\bfc_k)
\end{equation}
Higher score for $J(\bfC)$ indicates the better distinguishability between ID concept scores and OOD concept scores.
\end{enumerate}

Note the close relation to Fisher Linear Discriminant (FLD). FLD finds the optimal projection from high resolution input data into low dimensional representations that maximizes the separability between classes.
Let $\{\bfphi_1, \bfphi_2, .., \bfphi_n\}$ be $d$-dimensional samples that belong to one of binary classes, $y_i = \{0, 1\}$. \jihye{notation for detection vs notation for classification -- clarify!}
$\bfphi_i$ is the feature representation at layer $l$ flattened into $d$-dimensional vector: $\bfphi_i = \phi(\bfx_i)$.
Let $\bfv$ be a unit vector in the $d$-dimensional space and $z_i = \bfv\cdot\bfphi_i$ is the projection of $\bfphi_i$ into a one dimensional subspace.
Let $\mu_0 = \frac{1}{n_0}\sum_{z_i: y_i = 0}^{n_0} z_i = \bfv \cdot (\frac{1}{n_0}\sum_{\bfphi_i: y_i = 0}^{n_0} \bfphi_i)$ be the mean of projected values for class 0 and similarly, $\mu_1$ be the mean for class 1.
Define scatter for class 0 as $s_0 = \sum_{z_i: y_i = 0}^{n_0} (z_i - \mu_0)^2$ and similarly, $s_1$ is the scatter for class 1.
$s_0$ can be rewritten in a vector form as,
\begin{align*}
    s_0 &= \sum_{z_i: y_i = 0}^{n_0} (z_i - \mu_0)^2 = \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfv \cdot (\bfphi_i - \bfmu_0))^2 \\
    &= \bfv^\mathsf{T} \cdot \left \Big[ \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfphi_i - \bfmu_0) \cdot (\bfphi_i - \bfmu_0)^\mathsf{T} \right \Big] \cdot \bfv
\end{align*}
where $\bfmu_0 = \frac{1}{n_0}\sum_{\bfphi_i: y_i = 0}^{n_0} \bfphi_i$ is the sample mean for class 0.
Let $S_w$ be the within class scatter matrix: $S_w = \sum_{\bfphi_i: y_i = 0}^{n_0} (\bfphi_i - \bfmu_0) \cdot (\bfphi_i - \bfmu_0)^\mathsf{T} + \sum_{\bfphi_i: y_i = 1}^{n_1} (\bfphi_i - \bfmu_1) \cdot (\bfphi_i - \bfmu_1)^\mathsf{T}$. Then FLD measures the separability with respect to $\bfv$ as, 
\begin{equation}
    \label{equ: FLD}
    J_{Fisher}(\bfv) = \frac{(\mu_0 - \mu_1)^2}{(s_0 + s_1)} = \frac{\bfv^\mathsf{T} \cdot (\bfmu_0 - \bfmu_1)(\bfmu_0 - \bfmu_1)^\mathsf{T} \cdot \bfv }{\bfv^\mathsf{T} \cdot S_w \cdot \bfv}
\end{equation}
FLD finds $\widetilde{\bfv}$ such that $\frac{d J(\widetilde{\bfv})}{d \bfv} = 0$ for the optimal projection with maximum separability: $\widetilde{\bfv} = S_w^{-1}(\bfmu_0 - \bfmu_1)$.

Finally, our distinguishability index given a set of concept vectors $\bfC = \{\bfc_1, \bfc_2, ..., \bfc_m\}$ is defined as,
\begin{equation}
    \label{equ: distinguishability}
    S(\bfC) = \frac{J(\bfC)}{J_{Fisher}(\widetilde{\bfv})}
\end{equation}
% Guan et al. introduces Distance-based Separability Index (DSI) that measures how the distribution of intra-class distance (ICD) resembles the distribution of between-class distance (BCD) through statistical testing ~\cite{separability}. As the two classes are more separable, ICD and BCD are more distinguishable. 
% They verify the DSI to be more effective in measuring the separability of both synthetic and real-world datasets, compared to other separability indices such as Fisher discriminant ratio, neighborhood measures and linearity measures.
% We adopt DSI to quantify how distinguishable the ID concept scores and OOD concept scores are.
% Given $D_{\text{in}}^{test} = \{(\bfx_i, y_i)\}_{i=1}^{N_{in}}$ and $D_{\text{out}}^{test} = \{\bfx_i\}_{i=1}^{N_{out}}$, and a set of concept vectors $\bfC = \{\bfc\}_i^m$, we compute separability score between ID and OOD:
% \begin{enumerate}
%     \item First, we prepare $S_{in} = \{s_1, s_2, ..., s_{N_{in}}~|~s_i = v_\bfC(\bfx_i), \bfx_i \in D^{test}_{in}\}$ and $S_{out} = \{s_1, s_2, ..., s_{N_{out}}~|~s_i = v_\bfC(\bfx_i), \bfx_i \in D^{test}_{out}\}$. These are the set of concept scores for ID and OOD data, respectively.
    
%     \item ICD set for ID data, $\{d_{in}\}$ is a set of $l_2$ distances between any two points in $S(D_{\text{in}}^{test})$: $\{d_{in}\} = \{||s_i - s_j||_2 ~|~ s_i, s_j \in S_{in}; s_i \neq s_j\}$.
%     Likewise, $\{d_{out}\}$ is the ICD set for OOD data.
    
%     \item BCD set between ID and OOD data, $\{d_{in, out}\}$ is the set of $l_2$ distances between any two points from different distribution (ID and OOD): $\{d_{in, out}\} = \{||s_{in} - s_{out}||_2 ~|~ s_{in} \in S_{in}, s_out \in S_{out}\}$.
    
%     \item Then, the similarity between the ICD and BCD sets are computed using the Kolmogorov-Smirnov (KS) distance:
%     \[k_{in} = KS(\{d_{in}\}, \{d_{in, out}\}), \textrm{and}~ k_{out} = KS(\{d_{out}\}, \{d_{in, out}\})\]
%     \item Finally, the DSI of ID and OOD data is computed by averaging the two KS distances as follows,
%     \begin{equation}
%         \label{equ: separability}
%         DSI(D_{\text{in}}^{test}, D_{\text{out}}^{test}) = \frac{(k_{in} + k_{out})}{2}
%     \end{equation}
% \end{enumerate}

\fi


\subsection{Proposed Concept Learning Algorithm}
\label{sec:concept_learning}

In this section, we develop our proposed concept learning objective that aims to find a set of concepts $\bfC = \{\bfc_1, \bfc_2, ..., \bfc_m\}$ and a mapping $\bfg$ (parameterized by a neural network) that have the following properties: 1) high detection completeness w.r.t the given OOD detector; 2) high classification completeness w.r.t the DNN classifier; and 3) high separability in the concept-score space between detected-ID data and detected-OOD data.
% between the samples detected as ID and the samples detected as OOD by the detector. 

\mypara{Limitations of Prior Work.} 
We first discuss some notable existing works on concept learning, whose focus is on the classification problem.
% We first discuss the drawback of a notable existing works related to concept discovery. 
\citeauthor{kim2018tcav}, \citeauthor{ghorbani2019ace} and \citeauthor{yeh2019completeness} are post-hoc concept-discovery methods that find concept vectors in the space supported by the intermediate feature representations of in-distribution training data.
Unlike \cite{kim2018tcav} and \cite{ghorbani2019ace}, that do not support imposing required conditions in the concept discovery process, \cite{yeh2019completeness} devised a learning-based approach where classification completeness and the saliency of concepts are optimized via regularization.
More explicitly, the concept learning objective of \cite{yeh2019completeness} is
\begin{equation}
\label{equ: baseline}
    \argmax_{\bfC, \bfg} \expec_{(\bfx, y) \sim \Pin}\!\!\big[ \log h_y(\bfg(\VC(\bfx))) \big] ~+~ \lambda_{\textrm{expl}}\, R_{\textrm{expl}}(\bfC),
\end{equation}
where $\bfC$ and $\bfg$ are jointly optimized, and $R_{\textrm{expl}}(\bfC)$ is a regularization term used to ensure that the learned concept vectors have high spatial coherency and low redundancy (among themselves).
Specifically, the regularization term is
\begin{align}
\label{equ:regularizer_expl}
    R_{\textrm{expl}}(\bfC) ~&=~ \frac{1}{m\,K} \mysum_{k=1}^m \mysum_{\bfx^\prime \in T_{\bfc_k}} \langle \bfphi(\bfx^\prime), \bfc_k \rangle \nonumber \\
    &-~ \frac{1}{m \,(m - 1)} \mysum_{j=1}^m \mysum_{k=j + 1}^m \langle \bfc_j, \bfc_k \rangle.
\end{align}
where $T_{\bfc_k}$ is the set of $K$-nearest neighbor patches of the concept vector $\bfc_k$ from the ID training set $\Dintr$.

% \begin{figure}[tb]
% \vspace{1mm}
% \centering
% %\includegraphics[width=0.45\textwidth]{figures/completeness.png}
% \includegraphics[scale=0.24]{figures/distribution.png}
% %\vspace{-2mm}
% \caption{Blue line is the estimated density of outputs from $\calD$ given ID test data (AwA), and red line is that of OOD test data (SUN). DNN classifier is Inception-V3 trained with AwA dataset.
% \textbf{First row}: distributions of outputs from MSP detector \cite{hendrycks2016msp}. 
% \textbf{Second row}: distributions of outputs from Energy detector \cite{liu2020energy}.
% \textbf{Left}: Target distribution of $S(\bfx, \bff)$ in canonical world. 
% \textbf{Mid}: Distribution of $S(\bfx, \fcon)$ in concept world, using concepts learned by \cite{yeh2019completeness}.
% \textbf{Right}: Distribution of $S(\bfx, \fcon)$ in concept world, using concepts learned by our framework.}
% \vspace{-5mm}
% \label{fig:score-distribution}
% \end{figure}

\begin{figure}[tbp]
\centering
\subfloat[MSP, target \label{fig:distr_msp_target}]{\includegraphics[width=0.15\textwidth]{figures/distr_msp_target.jpg}}\hfill
\subfloat[MSP, baseline \label{fig:distr_msp_yeh}] {\includegraphics[width=0.15\textwidth]{distr_msp_yeh.jpg}}\hfill
\subfloat[MSP, ours \label{fig:distr_msp_ours}]{\includegraphics[width=0.15\textwidth]{figures/distr_msp_ours.jpg}} \\
\subfloat[Energy, target\label{fig:distr_energy_target}]{\includegraphics[width=0.15\textwidth]{figures/distr_energy_target.jpg}}\hfill
\subfloat[Energy, baseline \label{fig:distr_energy_yeh}] {\includegraphics[width=0.15\textwidth]{figures/distr_energy_yeh.jpg}}\hfill
\subfloat[Energy, ours\label{fig:distr_energy_ours}]{\includegraphics[width=0.15\textwidth]{figures/distr_energy_ours.jpg}}
\caption{Estimated density of $S(\bfx, \cdot)$ between the AwA test data (ID; blue) and the SUN dataset (OOD; red). DNN classifier is Inception-V3 and OOD detector is either MSP \cite{hendrycks2016msp} or \cite{liu2020energy}.
\textbf{Left}: Target distribution of $S(\bfx, \bff)$ in canonical world. 
\textbf{Mid}: Distribution of $\Scon(\bfx, \bff)$ in concept world, using concepts learned by \cite{yeh2019completeness}.
\textbf{Right}: Distribution of $\Scon(\bfx, \bff)$ in concept world, using concepts learned by our method.
For MSP, we set $\lambda_\textrm{mse} = 10, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ and for Energy, $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$.}
\label{fig:score-distribution}
\end{figure}

Unfortunately, there is a caveat with their approach.
Eqn. (\ref{equ: baseline}) may encourage the concepts to have high classification completeness score (defined in Eqn. (\ref{equ: completeness-classification})), but their concepts may fail to reduce the gap between canonical world and concept world genuinely. \ryan{By ensuring that they achieve an}
\textit{accurate reconstruction} of $\hat{\calZ}$
, the resulted concept scores would be sufficient enough to recover the accuracy of $\bff$ in expectation, but it is unclear whether the per-instance behavior of $\bff$ (and moreover, $\calD$ that runs based on $\bff$) is genuinely imitated.
To be more specific, $\bfC$ would be a set of $m$ principal vectors 
the set of concept vectors
$m$ unit vectors that fully span the space supported by $\{\bfphi(\bfx_1), \cdots, \bfphi(\bfx_{\Nintr})$.
usually not independent to each other (\eg concept "Greenery" is negatively related to concept "Sea").
have no guarantee on how \textit{accurate} the concepts are in explaining the classifier and the OOD detector.
% The reason we should care about in instance-level behavior of $\bff$ and $\calD$ in concept world is as follows. 
Besides, since the focus of \cite{yeh2019completeness} is initially confined to studying the utility of concepts for classifier with ID data, there is no guarantee for the utility of concepts for OOD detector explanations.

To illustrate with a real example, Figure \ref{fig:score-distribution} shows the distribution of $S(\bfx, \bff)$ and $\Scon(\bfx, \bff)$ on the AwA dataset (ID) and the SUN dataset (OOD).
We observe that $\Scon(\bfx, \bff)$ based on the concepts learned by \cite{yeh2019completeness} has a totally different distribution for OOD data, when compared to the target distribution of $S(\bfx, \bff)$ in canonical world (see Figure \ref{fig:distr_msp_target} and \ref{fig:distr_msp_yeh}).
Not only for OOD data, their concepts result in mismatched distribution of $\Scon(\bfx, \bff)$ also with ID data (see Figure \ref{fig:distr_energy_target} and Figure \ref{fig:distr_energy_yeh}). 
To this end, we propose a general framework for concept learning that complements the previous works by additionally imposing instance-level requirements for concepts, and taking OOD data and OOD detector into consideration.
% \begin{equation}
% \label{equ: baseline+l2}
%     \argmax_{\bfC, g} \, \text{log} \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] + \lambda_1 \cdot R_{coherency}(\bfC) + \lambda_2 \cdot
%     \expec_{\bfx \sim D_{train}^{in}}||\phi(\bfx) - \hat{\phi}_{g, \bfC}(\bfx))||_2
% \end{equation}
% \begin{equation}
% \label{equ: baseline+score}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) ~-~ \alpha \expec_{\bfx \sim D_{train}^{in}} (\mathcal{D}(h(\hat{\phi}_{g, \bfC}(\bfx))) - \mathcal{D}(f(\bfx)))^2
% \end{equation}

% Let $D^{train} = \{D_{\text{in}}^{train} \cup D_{\text{out}}^{train}\}$, and data is drawn as $(\bfx, s) \sim D^{train}$ where $s \in \{0, 1\}$ is the groundtruth label of OOD detection.
%
% \begin{equation}
% \label{equ: baseline+separability}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) ~+~ \beta \expec_{\bfx \sim D^{train}} J(\bfC)
% \end{equation}
%

\begin{algorithm}[t]
\caption{Learning concepts for OOD detector}
\label{alg:concept_learning}
\textbf{INPUT:} Entire training set $\Dtr = \{\Dintr, \Douttr\}$, entire validation set $\Dval = \{\Dinval, \Doutval\}$, classifier $\bff$, detector $\calD$; \\
\textbf{INITIALIZE:} Concept vectors $\bfC = [\bfc_1 ... \bfc_m]$ and parameters of mapping $g$; \\
\textbf{OUTPUT:} $\bfC$ and $g$;
\begin{algorithmic}[1]
  \STATE Identify threshold $\gamma$ for $\calD_\gamma(\bfx, \bff)$ on $\Dval$ at which true positive rate is $95\%$;
%   , and prepare $\widehat{\Dinval}$ and $\widehat{\Doutval}$;
  \FOR{$t = 0, 1, ... T$}
    \STATE Compute prediction accuracy using $\Dintr$ and $\bff$;
    \STATE Compute explainability of $\bfC$ with $\Dintr$ using Eqn. (\ref{equ:regularizer_expl});
	\STATE Compute difference of feature representation between canonical world and concept world using Eqn. (\ref{equ:regularizer_norm});
	\STATE Compute difference of detector outputs between canonical world and concept world using Eqn. (\ref{equ:regularizer_mse});
	\STATE Compute $V_{\textrm{in}}(\bfC)$~\footnotemark and $V_{\textrm{out}}(\bfC)$ using $\Dtr, \calD_\gamma(\cdot)$ and $\bfC$.
	Compute compute separability between $V_{\textrm{in}}(\bfC)$ and $V_{\textrm{out}}(\bfC)$ using Eqn. (\ref{eq:separability_trace}) or Eqn. (\ref{eq:separability_trace_per_class});
    \STATE Update $\bfC$ and $g$ using Eqn. (\ref{equ: concept learning})
  \ENDFOR
\end{algorithmic}
\end{algorithm}
\footnotetext{To make the dimension reduction in $V_{\textrm{in}}(\bfC) := \{\widetilde{v}_{\bfc_i}(\bfx) ~|~ \widetilde{v}_{\bfc_i}(\bfx) = \max_{p, q} |\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle|, \, \bfx \sim \Pin\} $ differential, we take a smooth approximation to the maximum via the \texttt{logsumexp} operation: $\max_{p, q} |\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle| \approx \frac{1}{\alpha}\sum_{p,q}\log(e^{\alpha |\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle|})$ as $\alpha \rightarrow \infty$. The same applies to $V_{\textrm{out}}(\bfC)$.}

\mypara{Concept Learning Objective.}
We suggest a simple design of regularization, inspired by recent works on transferring feature information from the teacher model to the student model \cite{hinton2015distilling,ba2014deep,zhou2018rocket}.
Recall that $\bfC$ projects the space spanned by original feature representations $\calZ$ to concept space, which is then mapped to the reconstructed space $\hat{\calZ}$ by $\bfg$.
Intuitively, to encourage the accurate reconstruction of $\hat{\calZ}$, we require that the distance between $\recphi(\bfx)$ and $\bfphi(\bfx)$ are minimized and push the detector to output\ryan{"and push the detector to output" => "and push towards the detector's output"?}
Hence, we include an additional regularization term that minimizes the squared $\ell_2$ distance between feature representations in $\calZ$ and $\hat{\calZ}$, and the mean squared error between . \jihye{intuition behind using only ID for norm term and usign both ID and OOD for mse term}
\begin{align}
\label{equ:regularizer_norm}
    J_{\textrm{norm}}(\bfC) ~&=~ \expec_{\bfx \sim \Dintr}||\bfphi(\bfx) - \recphi(\bfx)||^2 \\
    \label{equ:regularizer_mse}
    J_{\textrm{mse}}(\bfC) ~&=~ \expec_{\bfx \sim \Dtr} (S(\bfx, \bfh \circ \recphi) - S(\bfx, \bfh \circ \bfphi))^2
\end{align}
\jihye{update to distribution}

Furthermore, to enhance the interpretatbiliy of our concept-based explanations, we impose an additional criterion for the concepts: separability. As already discussed in Section \ref{sec:separability_score}, our proposed separability metric is tractable by gradient-based optimization and can be directly applied to learning objective as a regularization term.
With all regularization terms put together, our final concept learning objective becomes
\begin{align}
\label{equ: concept learning}
\argmax_{\bfC, g}\, &\expec_{(\bfx, y) \sim \Pin}\!\!\big[ \log h_y(\bfg(\VC(\bfx))) \big] ~+~ \lambda_{\textrm{expl}}\, R_{\textrm{expl}}(\bfC) \nonumber \\ 
    &-~ \lambda_{\textrm{mse}}\, J_{\textrm{mse}}(\bfC) ~-~ \lambda_{\textrm{norm}}\,J_{\textrm{norm}}(\bfC) \nonumber \\
    &+~ \lambda_{\textrm{sep}}~J_{\textrm{sep}}(\bfC)
\end{align}
We summarize our complete concept learning algorithm in Algorithm \ref{alg:concept_learning}.



%
% Note that using \begin{align} ... \end{align} is a better way that using \begin{array}
% \begin{equation}
% \label{equ: concept learning}
% \begin{array}{l}
%     \argmax_{\bfC, g} \, \log \proba_{(\bfx, y) \sim D^{train}_{in}}[\, h_{y}(\hat{\phi}_{g, \bfC}(\bfx))] ~+~ \lambda\, R_{coherency}(\bfC) \hspace{20mm} \\
%     -~ \alpha\, \expec_{\bfx \sim D^{train}}\mathcal{D}(h(\hat{\phi}_{g, \bfC}(\bfx))) - \mathcal{D}(f(\bfx)))^2 
%     ~+~ \beta\, \expec_{\bfx \sim D^{train}} J(\bfC) \\
%     -~ \gamma\, \expec_{\bfx \sim D^{train}}||\phi(\bfx) - \hat{\phi}_{g, \bfC}(\bfx))||_2
% \end{array}
% \end{equation}



==> backups/results_old.tex <==
\begin{table*}[tb]
    \centering
    \begin{adjustbox}{width=2\columnwidth,center}
		\begin{tabular}{l|l|l|c|c|c|c|c|c|c|c}
			\toprule
			\multirow{3}{0.02\linewidth}{OOD detector} & \multirow{3}{0.13\linewidth}{Hyperparameters} &
			\multirow{3}{0.07\linewidth}{ $\eta^{}_{\bff}(\bfC)$} & \multicolumn{8}{c}{OOD data} \\ \cline{4-11}
    		& & & \multicolumn{2}{c|}{\texttt{Places}} & \multicolumn{2}{c|}{\texttt{SUN}} & \multicolumn{2}{c|}{\texttt{Textures}} & \multicolumn{2}{c}{\texttt{iNaturalist}}\\ \cline{4-11}
    		& & & $\eta^{}_{\bff, S}(\bfC)$ & J_{\textrm{sep}}(\bfC, \bfC') & $\eta^{}_{\bff, S}(\bfC)$ & J_{\textrm{sep}}(\bfC, \bfC') & $\eta^{}_{\bff, S}(\bfC)$ & J_{\textrm{sep}}(\bfC, \bfC') & $\eta^{}_{\bff, S}(\bfC)$ & J_{\textrm{sep}}(\bfC, \bfC') \\ \hline \hline
			\multirow{4}{0.10\linewidth}{MSP} 
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$ & 0.990 & 0.849 & 0.0 & 0.848 & 0.0 & 0.824 & 0.0 & 0.958 & 0.0\\
			& $\lambda_\textrm{mse} = 10, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ & \textbf{0.994} & 0.947 &0.216 & 0.946 & 0.118 & 0.922 & \textbf{0.406} & \textbf{0.970} & 0.175 \\
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 50$ & 0.980 & 0.815 & \textbf{0.412} & 0.816 & \textbf{0.303} & 0.773 & 0.376 & 0.863 & 0.267\\
			& $\lambda_\textrm{mse} = 10, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$ & 0.985 & \textbf{0.959} & 0.327 & \textbf{0.961} & 0.266 & \textbf{0.938} & 0.344 & 0.946 & \textbf{0.286}\\ \hline 
			\multirow{4}{0.10\linewidth}{ODIN} 
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$ & 0.990 & 0.869 & 0.0 & 0.869 & 0.0 & 0.850 & 0.0 & 0.981 & 0.0\\
			& $\lambda_\textrm{mse} = 10^8, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ & \textbf{0.994} & 0.951 & 0.161 & 0.959 & 0.215 & 0.936 & 0.411 & 0.936 & 0.151\\
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 50$ & 0.987 & 0.899 & \textbf{0.373} & 0.911 & 0.342 & 0.790 & \textbf{0.414} & 0.970 & \textbf{0.337}\\
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$ & 0.991 & \textbf{0.973} & 0.355 & \textbf{0.969} & \textbf{0.356} & \textbf{0.945} & 0.405 & \textbf{0.982} & 0.308 \\ \hline
			\multirow{4}{0.10\linewidth}{Energy} 
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$ & 0.990 & 0.845 & 0.0 & 0.847 & 0.0 & 0.832 & 0.0 & 0.973 & 0.0\\
			& $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ & \textbf{0.993} & 0.965 & 0.135 & 0.963 & 0.127 & 0.960 & 0.284 & 0.949 & 0.215\\
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 50$ & 0.987 & 0.779 & \textbf{0.422} & 0.794 & 0.371 & 0.767 & \textbf{0.510} & 0.911 & \textbf{0.288} \\
			& $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$ & 0.990 & \textbf{0.971} & 0.365 & \textbf{0.970} & \textbf{0.400} & \textbf{0.964} & 0.494 & \textbf{0.973} & 0.280\\ \hline
			\multirow{4}{0.10\linewidth}{Mahal} 
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$ & 0.990 & 0.860 & 0.0 & 0.860 & 0.0 & 0.831 & 0.0 & 0.972 & 0.0 \\
			& $\lambda_\textrm{mse} = 0.1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ & \textbf{0.994} & 0.962 & 0.153 & 0.963 & 0.176 & 0.962 & 0.351 & 0.955 & 0.169\\
			& $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 50$ & 0.985 & 0.850 & \textbf{0.430} & 0.883 & 0.362 & 0.774 & \textbf{0.429} & 0.926 & \textbf{0.386} \\
			& $\lambda_\textrm{mse} = 0.1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$ & 0.991 & \textbf{0.971} & 0.370 & \textbf{0.970} & \textbf{0.388} & \textbf{0.970} & 0.397 & \textbf{0.972} & 0.351 \\ \bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small \textbf{Results of concept learning with different parameter settings across various OOD detectors and OOD datasets.} $\bfC'$ denotes a set of concepts discovered by baseline \cite{yeh2019completeness} (\ie $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$).
	Note that by definition of $J_{\textrm{sep}}(\bfC, \bfC')$ (Eqn. \ref{eq:relative-separability}), $J_{\textrm{sep}}(\bfC, \bfC') = 0$ for baseline.
	By having $\lambda_\textrm{mse} > 0, \lambda_\textrm{norm} > 0, \lambda_\textrm{sep} = 0$, we observe that $\eta^{}_{\bff, S}(\bfC)$ is always improved by large margin compared to baseline.
	When $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} > 0$, $J_{\textrm{sep}}(\bfC, \bfC')$ is maximized the most, but $\eta^{}_{\bff, S}(\bfC)$ is not enhanced or even degraded.
	Finally, with $\lambda_\textrm{mse} > 0, \lambda_\textrm{norm} > 0, \lambda_\textrm{sep} > 0$ when all of our regularization terms are considered, we achieve the best detection completeness in most of the cases.
	To encourage both detection completeness and concept separability, we have to sacrifice $J_{\textrm{sep}}(\bfC)$ a bit, but it is still a noticeable improvement compared to baseline.
	\textbf{Bold} numbers are superior results.}
	\label{tab:concept-learning-results}
\end{table*}

\section{Experiments}
\subsection{Setup}
\textbf{Dataset.} For the ID dataset, we use Animals with Attributes (AwA) \cite{xian2018awa} with 50 animal classes, and split it into train set (29841 images), validation set (3709 images), and test set (3772 images).
For OOD datasets, we use the MSCOCO dataset \cite{lin2014mscoco} as $\Douttr$.
For the OOD test dataset $\Doutte$ at test time, we follow a common setting in literature of large-scale OOD detection and use four different datasets: \texttt{Places365} \cite{zhou2017places}, \texttt{SUN} \cite{xiao2010sun}, \texttt{Textures} \cite{cimpoi2014textures}, \texttt{iNaturalist} \cite{van2018inaturalist}, all resized to $224 \times 224$ input shape.

% \jihye{real-world high resolution image data}
\textbf{DNN classifier.} To follow common setup in prior works \cite{yeh2019completeness, ghorbani2019ace, koh2020concept-bottleneck, kim2018tcav}, we test our method to interpret the widely-used Inception-V3 model \cite{szegedy2016inception-v3} trained on AwA, which yields $0.921$ test accuracy. 
For interpretation, we choose a layer right before the global max-pooling layer. 

\textbf{OOD detector.} We apply our general approach to intepret four popular OOD detection methods in the literature: MSP \cite{hendrycks2016msp}, ODIN \cite{liang2018ODIN}, Energy \cite{liu2020energy} and Mahalanobis \cite{lee2018mahalanobis} (henceforth abbreviated to Mahal). 

\textbf{Hyperparameters.}
In the following sections, all results are from applying different concept learning objectives to obtain $m = 100$ concepts (unless specifically mentioned otherwise). 
Following the implementation of \cite{yeh2019completeness}, we fix $\lambda_{\textrm{expl}} = 10$ throughout our experiments, set $\bfg$ to be a two-layer perceptron with $500$ neurons at hidden layer, and optimize using Adam \cite{kingma2014adam}.
We set the range of $\lambda_{\textrm{norm}}, \lambda_{\textrm{mse}}$ and $\lambda_{\textrm{sep}}$ (see Eqn. (\ref{equ: concept learning})) depending on the scale of corresponding terms (\ie $J_{\textrm{norm}}(\bfC),  J_{\textrm{mse}}(\bfC)$ and $ J_{\textrm{sep}}(\bfC)$, respectively) with a specific choice of OOD detector.
For ablation study to illustrate the effect of each parameter, see Appendix \ref{sec:appendix-concept-learning-ablation}\ryan{just adding a reminder to fill this in before submission}.
After concept learning with $m$ concepts, we remove duplicate concepts by removing those with a dot product of over $0.95$ with the others~\cite{yeh2019completeness}.

\subsection{Results}\label{subsec:results}
\mypara{Effectiveness of our concept learning objective.}
We test how effectively our regularization terms improve detection completeness and concept separability, without sacrificing the classification completeness.
In contrast to completeness scores that are close to the range $[0, 1]$ regardless of the choice of dataset, classification model or OOD detection algorithm, it is hard to gauge the possible range of separability score $J_{\textrm{sep}}(\bfC)$ (or $J^y_{\textrm{sep}}(\bfC)$) across different settings, and whether the resulted score is a meaningful improvement.
Hence, we devise a \textit{relative} concept separability that captures the relative improvement in concept separability between two different sets of concepts as
\begin{equation}
\label{eq:relative-separability}
J_{\textrm{sep}}(\bfC, \bfC') = \textrm{Median}\left(\left\{\frac{J^i_{\textrm{sep}}(\bfC) - J^i_{\textrm{sep}}(\bfC')}{J^i_{\textrm{sep}}(\bfC')}\right\}_{i=1}^L\right).   
\end{equation}
Eqn. (\ref{eq:relative-separability}) measures the median of the relative increase in the per-class separability $J^y_{\textrm{sep}}(\bfC)$ using concept $\bfC$, compared to $J^y_{\textrm{sep}}(\bfC')$ using another set of concept $\bfC'$.
We set $\bfC'$ to be the set of concepts learned by \cite{yeh2019completeness}, which is a special case of our learning objective when $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$.
The set of concept $\bfC$ can be obtained via our concept learning with various combinations of hyperparameter choices.
For the full results of relative separability along with classification completeness and detection completeness across various OOD detectors and OOD datasets, refer to Table \ref{tab:concept-learning-results}.

Table \ref{tab:concept-learning-results} shows that $J_{\textrm{norm}}(\bfC)$ and $J_{\textrm{mse}}(\bfC)$ regularizers not only encourage the detection completeness, but also the classification completeness as well. 
This verifies our assumption that accurate reconstruction of feature representation space $\hat{\calZ}$ is beneficial for accurate explanations for both classifier and OOD detector.
Moreover, by having the separability regularizer $J_{\textrm{sep}}(\bfC)$, we improve the detection completeness even further, with better relative concept separability as well.

\begin{figure}[tbp]
\centering
\subfloat[MSP, target \label{fig:distr_msp_target}]{\includegraphics[width=0.15\textwidth]{figures/distr_msp_target.jpg}}\hfill
\subfloat[MSP, baseline \label{fig:distr_msp_yeh}] {\includegraphics[width=0.15\textwidth]{distr_msp_yeh.jpg}}\hfill
\subfloat[MSP, ours \label{fig:distr_msp_ours}]{\includegraphics[width=0.15\textwidth]{figures/distr_msp_ours.jpg}} \\
\subfloat[Energy, target\label{fig:distr_energy_target}]{\includegraphics[width=0.15\textwidth]{figures/distr_energy_target.jpg}}\hfill
\subfloat[Energy, baseline \label{fig:distr_energy_yeh}] {\includegraphics[width=0.15\textwidth]{figures/distr_energy_yeh.jpg}}\hfill
\subfloat[Energy, ours\label{fig:distr_energy_ours}]{\includegraphics[width=0.15\textwidth]{figures/distr_energy_ours.jpg}}
\caption{Estimated density of $S(\bfx, \cdot)$ between the AwA test data (ID; blue) and the SUN dataset (OOD; red). DNN classifier is Inception-V3 and OOD detector is either MSP \cite{hendrycks2016msp} or \cite{liu2020energy}.
\textbf{Left}: Target distribution of $S(\bfx, \bff)$ in canonical world. 
\textbf{Mid}: Distribution of $\Scon(\bfx, \bff)$ in concept world, using concepts learned by \cite{yeh2019completeness}.
\textbf{Right}: Distribution of $\Scon(\bfx, \bff)$ in concept world, using concepts learned by our method.
For MSP, we set $\lambda_\textrm{mse} = 10, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$ and for Energy, $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$.}
\label{fig:score-distribution}
\end{figure}



\mypara{Reconstruction of $\hat{\calZ}$.}
% Other than observing increased detection completeness, 
To gain further insights on how accurately the feature representation space can be reconstructed from concept scores, we inspect the distribution of OOD detector scores in canonical world and concept world, using different sets of concepts (Figure \ref{fig:score-distribution}).
The distribution of $\Scon(\bfx, \bff)$ calculated based on concepts by baseline ($\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$) is significantly different from the target distribution of $S(\bfx, \bff)$ (see Figure \ref{fig:distr_msp_target} vs. Figure \ref{fig:distr_msp_yeh}, and Figure \ref{fig:distr_energy_target} vs. Figure \ref{fig:distr_energy_yeh}). This demonstrates that the concepts from~\cite{yeh2019completeness} may not directly match the distribution in either the ID or OOD data, and does not lead to optimal results in OOD detection.

In contrast, $\Scon(\bfx, \bff)$ (calculated based on concepts found by our method ($\lambda_\textrm{mse} > 0, \lambda_\textrm{norm} > 0, \lambda_\textrm{sep} = 0$)) approximates target distributions more closely for both ID and OOD data (see Figure \ref{fig:distr_msp_target} vs. Figure \ref{fig:distr_msp_ours}, and Figure \ref{fig:distr_energy_target} vs. Figure \ref{fig:distr_energy_ours}), showing the utility of our general concept explanation framework.
Overall, our experiments show that using the proposed regularization terms reduces the performance gap of both classifier and OOD detector in our two-world view, and and as a result, enables more accurate explanations for OOD detection.


\textbf{Transferability of concepts between OOD detectors.}
Our work essentially suggests to use different set of concepts for a specific target OOD detector, as $J_{\textrm{mse}}(\bfC)$ and $J_{\textrm{sep}}(\bfC)$ in Eqn. (\ref{equ: concept learning}) depend on a choice of OOD detector. 
In practice, however, one might not have enough computational capacity to prepare multiple sets of concepts for all type of OOD detectors at hand.
Here, we inspect the transferability of concepts across OOD detectors.
\begin{table}[htb]
    \small
    \centering
    \begin{adjustbox}{}
		\begin{tabular}{l|l|c|c|c|c}
			\toprule
			\multirow{2}{0.14\linewidth}{OOD data} & \multirow{2}{0.06\linewidth}{Metrics} & \multicolumn{4}{c}{OOD detector} \\ \cline{3-6}
    		& & MSP & ODIN & Energy & Mahal\\  \hline \hline
    % 		& & & $\mu_{f, \calD} (\bfC)$ & S(\bfC) & $\mu_{f, \calD} (\bfC)$ & S(\bfC) & $\mu_{f, \calD} (\bfC)$ & S(\bfC) & $\mu_{f, \calD} (\bfC)$ & S(\bfC) \\ \hline \hline
			\multirow{2}{0.08\linewidth}{Places} & $\eta^{}_{\bff, S}(\bfC)$ &0.956& 0.954 &0.971 & 0.954\\ 
			& $J_{\textrm{sep}}(\bfC, \bfC')$ & 0.417 & 0.415 &0.365& 0.410 \\\hline 
            \multirow{2}{0.08\linewidth}{SUN} & $\eta^{}_{\bff, S}(\bfC)$ &0.949& 0.948 &0.970& 0.950\\ 
			& $J_{\textrm{sep}}(\bfC, \bfC')$ & 0.355 &0.286 &0.400& 0.353 \\\hline 
			\multirow{2}{0.08\linewidth}{Textures} & $\eta^{}_{\bff, S}(\bfC)$ &0.931& 0.943 &0.964& 0.947\\ 
			& $J_{\textrm{sep}}(\bfC, \bfC')$ & 0.567 & 0.862&0.494&0.701 \\\hline 
			\multirow{2}{0.08\linewidth}{iNaturalist} & $\eta^{}_{\bff, S}(\bfC)$ &0.943& 0.939 &0.973& 0.940\\ 
			& $J_{\textrm{sep}}(\bfC, \bfC')$ & 0.283 &0.448 &0.280& 0.326\\
 \bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small \textbf{Transferability of concepts targeted for Energy with $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$}.}
	\label{tab:transferability-energy}
\end{table}
Table \ref{tab:transferability-energy} shows that concepts lead to the best detection completeness score when tested with the same type of OOD detector (\ie Energy). 
Interestingly, we can observe better concept separability with different type of OOD detectors.
For instance, with \texttt{Textures}, the best relative concept separability is achieved with ODIN detector (\ie $J_\textrm{sep}(\bfC, \bfC') = 0.862$) and which is even higher than the best results we could obtain using the set of concepts targeted for ODIN (\ie $J_\textrm{sep}(\bfC, \bfC') = 0.414$ with $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 50$ in Table \ref{tab:concept-learning-results}).
For full transferability results of concepts targeted for different type of OOD detectors, see Appendix \ref{sec:appendix-concept-learning-transfer}.

\subsection{Explanations}
In this subsection, we demonstrate how one can provide explanations for OOD detector given a set of concepts learned using our framework.
% \begin{itemize}
%     \item What set of the concepts is most prominent across the data detected as ID (or OOD) by $\mathcal{D}$?
%     \item What set of the concepts contribute to distinguish the ID and OOD data detected by $\mathcal{D}$?
%     \item How the change in concept score affects the $\mathcal{D}$'s detection result?
%     % \jihye{check perturbation generation in ATOM <-- permutation in concept space?}
% \end{itemize}

\begin{figure}[tb]
% \vspace{1mm}
\centering
%\includegraphics[width=0.45\textwidth]{figures/completeness.png}
\includegraphics[scale=0.28]{figures/expl_sheep.png}
\vspace{-9mm}
\caption{\small \textbf{Top-6 important concepts for Energy with respect to class "Sheep".}
Concepts are obtained by our concept learning algorithm with $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 0$.
To visualize what each concept represent, we display top receptive fields from $\Dinte$ whose inner product with the corresponding concept vector is above 0.8, along with the corresponding $\textrm{SHAP}(\eta^{j}_{\bff, S}, \bfc_i)$ value.}
\vspace{-5mm}
\label{fig:shap_sheep}
\end{figure}
\mypara{Contribution of each concept to detection.}
We address the following question: \textit{how much each concept contributes to OOD detection result?}
Recent works have suggested to adopt Shapley value from coalitional game theory literature \cite{shapley1953value,fujimoto2006axiomatic} to interpreting model predictions \cite{chen2018shapley,lundberg2017shapley,sundararajan2020shapley}.
Extending the idea, we modify Shapley value by incorporating our detection completeness metric (Eqn. (\ref{equ: completeness-detection})) as
\begin{align}
    \label{equ: ConceptSHAP}
    &\textrm{SHAP}(\eta^{}_{\bff, S}, 
    \bfc_i)  ~:= \nonumber \\
    &\sum_{\bfC' \subseteq \bfC \setminus \bfc_i} \frac{(m - |\bfC'| - 1)! |\bfC'|!}{m!} [\eta^{}_{\bff, S}(\bfC' \cup \{\bfc_i\}) - \eta^{}_{\bff, S}(\bfC')]
\end{align}
where $\bfC'$ is the subset of $\bfC$, and a high value represents the average marginal contribution of $\bfc_i$ across all possible coalitions when all classes are considered.
However, one might also want to assess the contribution of concepts to detection with respect to a particular class like "\textit{what concepts attribute to different detection results among the inputs predicted to the same class?}"
Thus, we can simply modify our detection completeness definition (Definition. (\ref{def:completeness_detec}) into its per-class variation by considering data that belong to a specific class $j$ as follows,
\begin{definition}
\label{def:completeness_detec_perclass}
Given a trained DNN classifier $\bff = \bfh \circ \bfphi$, a trained OOD detector with score function $S(\bfx, \bff)$, and a set of concept vectors $\bfC$, the {\em detection completeness score} with respect to ID distribution $\Pin(\bfx, y)$ and OOD distribution $\Pout(\bfx)$ is defined as
\begin{align}
\label{equ: completeness-detection-perclass}
    \eta^{j}_{\bff, S}(\bfC) 
    ~:=~ \frac{\textrm{sup}_\bfg \,\textrm{AUC}(\bfh \circ \recphi) ~-~ b_r}{\textrm{AUC}(\bfh \circ \bfphi) ~-~ b_r},
\end{align}
\end{definition}
% Note that for numerator we use predicted label -- don't have labels for OOD data. 
Accordingly, we use SHAP($\eta^{j}_{\bff, S}(\bfC)$) to denote SHAP($\eta^{}_{\bff, S}(\bfC) $) score specific to class $j$ where $\eta^{}_{\bff, S}(\bfC)$ is replaced in Eqn. (\ref{equ: completeness-detection-perclass}).
We show the top-ranked concepts by SHAP($\eta^{j}_{\bff, S}(\bfC)$) with respect to a specific class prediction in Figure \ref{fig:shap_sheep} (see Appendix \ref{sec:appendix-shapleys} for more results).
Also, we further investigate the attribution of such top-ranked concepts via counterfactual analysis (Appendix \ref{sec:appendix-counterfactual}).



% \mypara{Separability and interpretatbility}
% \begin{figure*}
%   \centering
%   \begin{tabular}{cc}
%     \subfloat[\label{fig:mnist}][Sampling distribution is skewed consistently for a single class (i.e. class 0)]
%     {
%     \hspace{-5mm}
%     \includegraphics[width=.49\linewidth]{mnist_class_0}} 
%     ~&~
%     \subfloat[\label{fig:asd}][Sampling distribution is skewed for the classes in turn (i.e. class 0, 1, 2, ...)]
%     {\includegraphics[width=.49\linewidth]{mnist_class_all}}
%   \end{tabular}
%   \caption{Accuracy vs training time-step in MNIST}
% \label{fig:mnist_results}
% \end{figure*}

\begin{figure*}[bt]
\centering
\subfloat[Set 1 with low concept separability, detected-ID \label{fig:low_in}]{\includegraphics[width=0.45\textwidth]{yeh_class17_AwA2_top10_detected_Energy.jpg}}\hfill
\subfloat[Set 2 with high concept separability, detected-ID \label{fig:high_in}] {\includegraphics[width=0.45\textwidth]{figures/ours_class17_AwA2_top10_detected_Energy.jpg}}\hfill\\
\vspace{-2mm}
\subfloat[Set 1 with low concept separability, detected-OOD \label{fig:low_out}]{\includegraphics[width=0.45\textwidth]{figures/yeh_class17_SUN_top10_detected_Energy.jpg}}\hfill
\subfloat[Set 2 with high concept separability, detected-OOD \label{fig:high_out}] {\includegraphics[width=0.45\textwidth]{figures/ours_class17_SUN_top10_detected_Energy.jpg}}
\caption{\small \textbf{Our concept separability metric and visual distinction in concept score patterns.} For class "Giraffe", we compare concept score patterns using different sets of concepts. \textbf{Left:} Averaged concept scores using concept set 1. \textbf{Right:} Averaged concept scores using concept set 2. For visualization of what each concept represents, see Appendix.}
\label{fig:high_separa_interpretatbility}
\end{figure*}
\mypara{Separability and interpretability}
Lastly, we use the concepts to gain insights on OOD detectors.
As shown in Figure \ref{fig:high_separa_interpretatbility}, we take the average of concept scores $V_{\textrm{in}}(\bfC')$ (or $V_{\textrm{out}}(\bfC')$) among the inputs that are predicted to class $j$, and detected as ID (or OOD) by OOD detector (\eg Energy in Figure \ref{fig:high_separa_interpretatbility}), where $\bfC'$ is the subset of original $m$ concepts $\bfC$. 
Here, we constitute the subset by taking the top-10 important concepts, ranked by their SHAP($\eta^{j}_{\bff, S}(\bfC)$) scores.
By comparing the patterns of averaged concept scores, one can understand how ID-detected inputs and OOD-detected inputs are different in terms of concepts, even when predicted to same class (compare Figure \ref{fig:low_in} vs. Figure \ref{fig:low_out}, or Figure \ref{fig:high_in} vs. Figure \ref{fig:high_out}).
Moreover, we confirm that a higher score for our concept separability metric enables more visual distinction  between concept score patterns.
For example, using concepts that yield relatively low per-class concept separability, $J^y_{\textrm{sep}}(\bfC')=0.059$, we fail to observe any noticeable difference in explanations between ID- and OO-detected data (see Figure \ref{fig:low_in} and \ref{fig:low_out}). 
On the other hand, concepts with high per-class concept separability, $J^y_{\textrm{sep}}(\bfC')=0.098$ successfully shows distinguishable pattern between ID- and OO-detected data (see Figure \ref{fig:high_in} and \ref{fig:high_out}). 
Such observation confirms our assumption that as long as classification completeness and detection completeness are preserved, having higher concept separability is beneficial for better interpretability for humans.
For further discussion, see Appendix \ryan{adding reminder to fill this in}.


==> contents/04_results_old.tex <==
\section{Experiments}
\label{subsec:results}

\iffalse

\begin{table*}[tb]
    \centering
    \begin{adjustbox}{width=1\columnwidth,center}
		\begin{tabular}{l|l|l|c|c|c|c|c|c|c|c}
			\toprule
			\multirow{3}{0.001\linewidth}{OOD detector} & \multirow{3}{0.10\linewidth}{Hyper-\\parameters} &
			\multirow{3}{0.05\linewidth}{ $\eta^{}_{\bff}(\bfC)$} & \multicolumn{8}{c}{OOD data} \\ \cline{4-11}
    		& & & \multicolumn{2}{c|}{\texttt{Places}} & \multicolumn{2}{c|}{\texttt{SUN}} & \multicolumn{2}{c|}{\texttt{Textures}} & \multicolumn{2}{c}{\texttt{iNaturalist}}\\ \cline{4-11}
    		& & & $\eta^{}_{\bff, S}(\bfC)$ & $J_{\textrm{sep}}(\bfC, \bfC')$ & $\eta^{}_{\bff, S}(\bfC)$ & $J_{\textrm{sep}}(\bfC, \bfC')$ & $\eta^{}_{\bff, S}(\bfC)$ & $J_{\textrm{sep}}(\bfC, \bfC')$ & $\eta^{}_{\bff, S}(\bfC)$ & $J_{\textrm{sep}}(\bfC, \bfC')$ \\ \hline \hline
			\multirow{4}{0.10\linewidth}{MSP \\ \citep{hendrycks2016msp}} 
			& $(0, 0, 0)$ & 0.977 \pm 0.0006 & 0.774 \pm 0.001 & 0.694 \pm 0.0153 & 0.782 \pm 0.001 & 1.088 \pm 0.0175 & 0.593 \pm 0.0013 & 0.765 \pm 0.0157 & 0.878 \pm 0.0008 & 1.075 \pm 0.0191\\
			& $(10, 0.1, 0)$ & \textbf{0.994} \pm 0.0004 & 0.947 \pm 0.0004 & 1.892 \pm 0.0393 & 0.946 \pm 0.0004 & 3.074 \pm 0.0531 & 0.920 \pm 0.0005 & 3.577 \pm 0.1292 & \textbf{0.967} \pm 0.0004 &  \\
			& $(0, 0, 50)$ & 0.980 \pm 0.0005 & 0.814 \pm 0.0008 & 2.533 \pm 0.0714 & 0.816 \pm 0.0009 & 4.295 \pm 0.1048 & 0.773 \pm 0.0010 & 3.147 \pm 0.2076 & 0.864 \pm 0.0007 &\\
			& $(10, 0.1, 50)$ & 0.984 \pm 0.0004 & \textbf{0.960} \pm 0.0004 & 2.756 \pm 0.0854 & \textbf{0.961} \pm 0.0005 & 4.442 \pm 0.0830 & \textbf{0.937} \pm 0.0004 & \textbf{0.439} \pm 0.0175 & 0.946 \pm 0.0004 & \textbf{0.795} \pm 0.0473\\ \hline 
			\multirow{4}{0.10\linewidth}{ODIN \\ \citep{liang2018ODIN}} 
			& $(0, 0, 0)$ & 0.977 \pm 0.0006 & 0.742 \pm 0.0011 & 0.0 & 0.745 \pm 0.0010 & 0.0 & 0.618 \pm 0.0013 & 0.0 & 0.906 \pm 0.0007 & 0.0\\
			& $(\expnum{1}{+8}, 0.1, 0)$ & \textbf{0.994} \pm 0.0004 & 0.951 \pm 0.0004 & -0.118 \pm 0.0099 & 0.958 \pm 0.0004 & -0.054 \pm 0.0119 & 0.934 \pm 0.0004 & -0.245 \pm 0.0133 & 0.935 \pm 0.0004 & -0.345 \pm 0.0153\\
			& $(0, 0, 50)$ & 0.987 \pm 0.0004 & 0.899 \pm 0.0007 & \textbf{0.492} \pm 0.0215 & 0.911 \pm 0.0006 & 0.520 \pm 0.0187 & 0.793 \pm 0.0008 & 0.422 \pm 0.0175 & 0.971 \pm 0.0004 & 0.318 \pm 0.0343\\
			& $(\expnum{1}{8}, 0.1, 50)$ & 0.991 & \textbf{0.973} & 0.355 & \textbf{0.969} & \textbf{0.356} & \textbf{0.945} & 0.405 & \textbf{0.982} & 0.308 \\ \hline
			\multirow{4}{0.10\linewidth}{General-ODIN \\ \citep{hsu2020GeneralizedODIN}} 
			& $(0, 0, 0)$ & 0.990 \pm 0.0004 & 0.869 & 0.0 & 0.869 & 0.0 & 0.850 & 0.0 & 0.981 & 0.0\\
			& $(10^8, 0.1, 0)$ & \textbf{0.994} \pm 0.0004 & 0.951 \pm 0.0006 & 0.161 & 0.959 & 0.215 & 0.936 & 0.411 & 0.936 & 0.151\\
			& $(0, 0, 50)$ & 0.987 & 0.899 & \textbf{0.373} & 0.911 & 0.342 & 0.790 & \textbf{0.414} & 0.970 & \textbf{0.337}\\
			& $(10^8, 0.1, 50)$ & 0.991 & \textbf{0.973} & 0.355 & \textbf{0.969} & \textbf{0.356} & \textbf{0.945} & 0.405 & \textbf{0.982} & 0.308 \\ \hline
			\multirow{4}{0.10\linewidth}{Energy \\ \citep{liu2020energy}} 
			& $(0, 0, 0)$ & 0.977 \pm 0.0006 & 0.671 \pm 0.0012 & 0.0 & 0.682 \pm 0.0012 & 0.0 & 0.557 \pm 0.0014 & 0.0 & 0.871 \pm 0.0007 & 0.0\\
			& $(1. 0.1, 0)$ & \textbf{0.993} \pm 0.0005 & \textbf{0.965} \pm 0.0004 & 0.191 \pm 0.0126 & \textbf{0.963} \pm 0.0004 & 0.326 \pm 0.0133 & \textbf{0.960} \pm 0.0003 & 0.110 \pm 0.0117 & \textbf{0.949} \pm 0.0004 & 0.770 \pm 0.0334\\
			& $(0, 0, 50)$ & 0.987 \pm 0.0005 & 0.779 \pm 0.0010 & 0.4703 \pm 0.0199 & 0.793 \pm 0.0009 & 0.427 \pm 0.0153 &  0.767 \pm 0.0010 & 0.531 \pm 0.0184 & 0.911 \pm 0.0006 & 0.263 \pm 0.0297 \\
			& $(1, 0.1, 50)$ & 0.980 \pm 0.0005 & 0.943 \pm 0.0005 & 0.534 \pm 0.0218 & \textbf{0.941} \pm 0.0005 & 0.534 \pm 0.0175 & 0.936 \pm 0.0005 & 0.658 \pm 0.0212 & 0.927 \pm 0.0005 & 0.291 \pm 0.0319 \\ \hline
			\multirow{4}{0.10\linewidth}{Mahal \\ \citep{lee2018mahalanobis}} 
			& $(0, 0, 0)$ & 0.990 & 0.860 & 0.0 & 0.860 & 0.0 & 0.831 & 0.0 & 0.972 & 0.0 \\
			& $(0.1, 0.1, 0)$ & \textbf{0.994} & 0.962 & 0.153 & 0.963 & 0.176 & 0.962 & 0.351 & 0.955 & 0.169\\
			& $(0, 0, 50)$ & 0.985 & 0.850 & \textbf{0.430} & 0.883 & 0.362 & 0.774 & \textbf{0.429} & 0.926 & \textbf{0.386} \\
			& $(0.1, 0.1, 50)$ & 0.991 & \textbf{0.971} & 0.370 & \textbf{0.970} & \textbf{0.388} & \textbf{0.970} & 0.397 & \textbf{0.972} & 0.351 \\ \bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{\small \textbf{Results of concept learning with different parameter settings across various OOD detectors and OOD datasets.} 
% 	$\bfC'$ denotes a set of concepts discovered by baseline \citep{yeh2020completeness} (\ie $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$).
	Hyperparameters are in the order of $(\lambda_\textrm{mse}, \lambda_\textrm{norm}, \lambda_\textrm{sep})$. Larger values are better for all the metrics. \textbf{Bold} numbers indicate the best results (across the rows) for a given OOD detection method and dataset. Note that by definition of $J_{\textrm{sep}}(\bfC, \bfC')$ (Eqn. \ref{eq:relative-separability}), the relative concept separability of the baseline~\citep{yeh2020completeness} is always $0$, \ie $J_{\textrm{sep}}(\bfC', \bfC') = 0$.}
	\label{tab:concept-learning-results}
\end{table*}

\fi

\iffalse

We perform experiments to evaluate the proposed method and address the following questions:
\begin{enumerate}[start=1,label={\bfseries Q\arabic*.}]
    \item \label{Q1} Does our concept learning objective effectively encourage concepts to have the desired properties of detection completeness and concept separability?
    \item \label{Q2} Are the proposed evaluation metrics well-aligned with the interpretability of the resulting concept-based explanations?
    % Are the proposed evaluations metrics beneficial for better interpretability of resulting concept-based explanations?
    % \jayaram{Are the proposed evaluation metrics effective at providing better interpretability for the resulting concept-based explanations?}
    % Does a high detection completeness score of concepts imply a more accurate explanaation of the OOD detector? Does better concept separability lead to a more distinctive explanation between ID- and OOD-detected data?
    \item \label{Q3} Given concepts learned by our approach, what insights can we provide for the OOD detector?
\end{enumerate}

Our main findings are summarized as follows:
\begin{enumerate}[start=1,label={\bfseries A\arabic*.}]
    \item In accordance with our design intention, our $\ell_2$ norm-based regularization and MSE regularization not only improve the detection completeness by large margin, but also the classification completeness even further. 
    The proposed separability regularization effectively improves concept separability, and when these three terms are used together in concept learning objective, we can achieve the highest detection completeness and concept separability (see Table \ref{tab:concept-learning-results}).
    \item Concepts with a high completeness score enable to mimic the original behavior of the OOD detector more precisely, hence leading to more \textit{accurate} explanations based on the concepts (see Fig. \ref{fig:score-distribution}). 
    Also, concepts with a higher concept separability score lead to more \textit{visually-distinctive} interpretations between ID and OOD data by having more distinguishable concept-score patterns (see Fig. \ref{fig:high_separa_interpretatbility}).
    % Concepts learned by our method enable more \textit{accurate}, and more \textit{visually distinctive} interpretations, compared to the concepts learned by the baseline method (\citep{yeh2020completeness}).
    \item We can rank the importance of each concept towards OOD detection using the Shapley value modified with our per-class detection completeness metric. 
    When the concepts are only targeted at explaining the DNN classifier (as in the baseline \citep{yeh2020completeness}), the behavior of the OOD detector is merely described by the common set of concepts that are important for the DNN classifier.
    On the other hand, when not only the DNN classifier but also the OOD detector is taken into consideration during concept learning (\ie our method), we obtain a more diverse and expanded set of concepts, and different concepts play a major role in interpreting the classification and detection results (see Fig. \ref{fig:shap_buffalo}). 
    % identify based on what concepts an OOD detector makes decisions.
    % We can identify the top concepts that contribute to the OOD detector's decisions using  
\end{enumerate}

\fi

% \subsection{Setup}\label{sec:setup}
We briefly describe the experimental setup here and provide additional details in Appendix \ref{sec:appendix-implementation-details}.
% We briefly describe the setup of our experiments to address the above questions. See Appendix \ref{sec:appendix-implementation-details} for further details.
% For reproducibility, we have released our anonymized source code ~\footnote{\url{https://anonymous.4open.science/r/Concept-For-OOD-CE1B/}}.

\mypara{Datasets.} For the ID dataset, we use Animals with Attributes (AwA) \citep{xian2018awa} with 50 animal classes, and split it into a train set (29841 images), validation set (3709 images), and test set (3772 images).
We use the MSCOCO dataset \citep{lin2014mscoco} as the auxiliary OOD dataset $\Douttr$ for training and validation.
For the OOD test dataset $\Doutte$, we follow a common setting in the literature of large-scale OOD detection \citep{Huang_MOS} and use three different image datasets: \texttt{Places365} \citep{zhou2017places}, \texttt{SUN} \citep{xiao2010sun}, and \texttt{Textures} \citep{cimpoi2014textures}.
% , \texttt{iNaturalist} \citep{van2018inaturalist}; all resized to the input size $224 \times 224$.

% \textbf{OOD detector.} We apply our general approach to intepret four popular OOD detection methods in the literature: MSP \citep{hendrycks2016msp}, ODIN \citep{liang2018ODIN}, Energy \citep{liu2020energy} and Mahalanobis \citep{lee2018mahalanobis} (henceforth abbreviated to Mahal).

% \jihye{real-world high resolution image data}
% \textbf{DNN classifier.} The OOD detectors are paired with the widely-used Inception-V3 model \citep{szegedy2016inception-v3} (following the common setup in prior works \citep{yeh2020completeness, ghorbani2019ace, koh2020concept-bottleneck, kim2018tcav}) trained on AwA, which yields $0.921$ test accuracy. 


\mypara{Models.}
We apply our framework to interpret five prominent OOD detectors from the literature: MSP~\citep{hendrycks2016msp}, ODIN~\citep{liang2018ODIN}, Generalized-ODIN~\citep{hsu2020GeneralizedODIN}, Energy~\citep{liu2020energy} and Mahalanobis~\citep{lee2018mahalanobis}.
The OOD detectors are paired with the widely-used Inception-V3 model~\citep{szegedy2016inception-v3} (following the setup in prior works~\citep{yeh2020completeness, ghorbani2019ace, kim2018tcav}) trained on the Animals-with-Attributes (AwA) dataset~\citep{xian2018awa}, which has a test accuracy of $92.10 \%$. 

\mypara{Metrics.}
For each set of concepts learned with different OOD detectors and hyperparameters, we report the classification completeness $\eta^{}_{\bff}(\bfC)$, detection completeness $\eta^{}_{\bff, S}(\bfC)$, and the relative concept separability metric (defined below). 
In contrast to the completeness scores that are almost always bounded to the range $[0, 1]$, it is hard to gauge the possible range of the separability score $J_{\textrm{sep}}(\bfC)$ (or $J^y_{\textrm{sep}}(\bfC)$) across different settings (datasets, classification models, and OOD detectors), and whether the value represents a significant improvement in separability.
Hence, we define the \textit{relative concept separability}, which captures the relative improvement in concept separability using concepts $\bfC$ compared to a different set of concepts $\bfC'$, as follows
% between two different sets of concepts, as follows
% \vspace{-1mm}
\begin{equation}
\label{eq:relative-separability}
J_{\textrm{sep}}(\bfC, \bfC') = \textrm{Median}\left( \left\{\frac{J^y_{\textrm{sep}}(\bfC) ~-~ J^y_{\textrm{sep}}(\bfC')}{J^y_{\textrm{sep}}(\bfC')}\right\}_{y=1}^L \right).   
\end{equation}
% This metric measures the median of the relative increase in the per-class separability using concepts $\bfC$, compared to that of using a different set of concepts $\bfC'$.
We choose $\bfC'$ to be the set of concepts learned by the baseline~\citep{yeh2020completeness}, which is a special case of our learning objective when $\,\lambda_\textrm{mse} = \lambda_\textrm{norm} = \lambda_\textrm{sep} = 0$.
The set of concept $\bfC$ are obtained via our concept learning objective, with various combinations of hyperparameter values.

\begin{table*}[htb]
    \centering
    % \begin{adjustbox}{width=1\columnwidth,center}
    \begin{adjustbox}{width=1\textwidth,center}
		\begin{tabular}{l|l|l|c|c|c|c|c|c}
			\toprule
			\multirow{3}{0.001\linewidth}{OOD detector} & \multirow{3}{0.10\linewidth}{Hyper-\\parameters} &
			\multirow{3}{0.05\linewidth}{ $\eta^{}_{\bff}(\bfC) \uparrow$} & \multicolumn{6}{c}{Test OOD dataset} \\ \cline{4-9}
    		& & & \multicolumn{2}{c|}{\texttt{Places}} & \multicolumn{2}{c|}{\texttt{SUN}} & \multicolumn{2}{c}{\texttt{Textures}}\\ \cline{4-9}
    		& & & $\eta^{}_{\bff, S}(\bfC) \uparrow$ & $J_{\textrm{sep}}(\bfC, \bfC') \uparrow$ & $\eta^{}_{\bff, S}(\bfC) \uparrow$ & $J_{\textrm{sep}}(\bfC, \bfC') \uparrow$ & $\eta^{}_{\bff, S}(\bfC) \uparrow$ & $J_{\textrm{sep}}(\bfC, \bfC') \uparrow$ \\ \hline \hline
			%
            \multirow{4}{0.10\linewidth}{MSP} 
			& $(0, 0, 0)$ & 0.977 $\pm$ 0.0006 & 0.774 $\pm$ 0.0010 & 0.694 $\pm$ 0.0153 & 0.782 $\pm$ 0.0010 & 1.088 $\pm$ 0.0175 & 0.593 $\pm$ 0.0013 & 0.765 $\pm$ 0.0157\\
			& $(10, 0.1, 0)$ & \underline{\textbf{0.994}} $\pm$ 0.0004 & \underline{0.947} $\pm$ 0.0004 & 1.892 $\pm$ 0.0393 & \underline{0.946} $\pm$ 0.0004 & 3.074 $\pm$ 0.0531 & \underline{0.920} $\pm$ 0.0005 & \underline{3.577} $\pm$ 0.1292\\
			& $(0, 0, 50)$ & 0.980 $\pm$ 0.0005 & 0.814 $\pm$ 0.0008 & \underline{2.533} $\pm$ 0.0714 & 0.816 $\pm$ 0.0009 & \underline{4.295} $\pm$ 0.1048 & 0.773 $\pm$ 0.0010 & 3.147 $\pm$ 0.2076\\
			& $(10, 0.1, 50)$ & \underline{0.984} $\pm$ 0.0004 & \underline{\textbf{0.960}} $\pm$ 0.0004 & \underline{\textbf{2.756}} $\pm$ 0.0854 & \underline{\textbf{0.961}} $\pm$ 0.0005 & \underline{\textbf{4.442}} $\pm$ 0.0830 & \underline{\textbf{0.937}} $\pm$ 0.0004 & \underline{\textbf{3.587}} $\pm$ 0.2145\\ \hline
			%
            \multirow{4}{0.10\linewidth}{ODIN} 
			& $(0, 0, 0)$ & 0.977 $\pm$ 0.0006 & 0.742 $\pm$ 0.0011 & 0.444 $\pm$ 0.0119 & 0.745 $\pm$ 0.0010 & 0.710 $\pm$ 0.0156 & 0.618 $\pm$ 0.0013 & 0.501 $\pm$ 0.0121 \\
			& $(10^8, 0.1, 0)$ & \underline{\textbf{0.994}} $\pm$ 0.0004 & \underline{0.951} $\pm$ 0.0004 & 1.166 $\pm$ 0.0303 & \underline{0.958} $\pm$ 0.0004 & 2.135 $\pm$ 0.0450 & \underline{0.934} $\pm$ 0.0004 & 2.793 $\pm$ 0.0865\\
			& $(0, 0, 50)$ & 0.987 $\pm$ 0.0004 & 0.899 $\pm$ 0.0007 & \underline{1.785} $\pm$ 0.0669 & 0.911 $\pm$ 0.0006 & \underline{3.814} $\pm$ 0.0768 & 0.793 $\pm$ 0.0008 & \underline{3.046} $\pm$ 0.2845\\
			& $(10^8, 0.1, 50)$ & \underline{0.991} $\pm$ 0,0005 & \underline{\textbf{0.973}} $\pm$ 0.0009 & \underline{\textbf{1.813}} $\pm$ 0.0268 & \underline{\textbf{0.969}} $\pm$ 0.0010 & \underline{\textbf{4.000}} $\pm$ 0.0094 & \underline{\textbf{0.945}} $\pm$ 0.0006 & \underline{\textbf{3.662}} $\pm$ 0.1005\\ \hline
			%
            \multirow{4}{0.10\linewidth}{General-ODIN} 
			& $(0, 0, 0)$ & 0.988 $\pm$ 0.0004 & 0.769 $\pm$ 0.0004 & 0.506 $\pm$ 0.0165 & 0.719 $\pm$ 0.0014 & 0.816 $\pm$ 0.0192 & 0.605 $\pm$ 0.0013 & 0.558 $\pm$ 0.1683\\
			& $(10^6, 0.1, 0)$ & \underline{\textbf{0.995}} $\pm$ 0.0004 & \underline{0.951} $\pm$ 0.0006 & 1.461 $\pm$ 0.0321 & \underline{0.960} $\pm$ 0.0005 & 3.007 $\pm$ 0.0316 & \underline{0.940} $\pm$ 0.0008 & 2.619 $\pm$ 0.1077\\
			& $(0, 0, 50)$ & 0.981 $\pm$ 0.0004 & 0.859 $\pm$ 0.0007 & \underline{1.814} $\pm$ 0.0685 & 0.803 $\pm$ 0.0006 & \underline{4.204} $\pm$ 0.0159 & 0.826 $\pm$ 0.0008 & \underline{\textbf{4.014}} $\pm$ 0.2246\\
			& $(10^6, 0.1, 50)$ & \underline{0.990} $\pm$ 0.0005 & \underline{\textbf{0.971}} $\pm$ 0.0010 & \underline{\textbf{1.835}} $\pm$ 0.0669 & \underline{\textbf{0.963}}$\pm$ 0.0004 & \underline{\textbf{4.287}} $\pm$ 0.0284 & \underline{\textbf{0.951}} $\pm$ 0.0005 & \underline{3.695} $\pm$ 0.1921 \\ \hline
			%
            \multirow{4}{0.10\linewidth}{Energy} 
			& $(0, 0, 0)$ & 0.977 $\pm$ 0.0006 & 0.671 $\pm$ 0.0012 & 0.453 $\pm$ 0.0121 & 0.682 $\pm$ 0.0012 & 0.675 $\pm$ 0.0148 & 0.557 $\pm$ 0.0014 & 0.521 $\pm$ 0.0131\\
			& $(1. 0.1, 0)$ & \underline{\textbf{0.993}} $\pm$ 0.0005 & \underline{\textbf{0.965}} $\pm$ 0.0004 & 1.266 $\pm$ 0.0319 & \underline{\textbf{0.963}} $\pm$ 0.0004 & 2.125 $\pm$ 0.0413 & \underline{\textbf{0.960}} $\pm$ 0.0003 & 2.648 $\pm$ 0.0596\\
			& $(0, 0, 50)$ & \underline{0.987} $\pm$ 0.0005 & 0.779 $\pm$ 0.0010 & \underline{\textbf{1.920}} $\pm$ 0.0725 & 0.793 $\pm$ 0.0009 & \underline{\textbf{3.659}} $\pm$ 0.0659 & 0.767 $\pm$ 0.0010 & \underline{\textbf{4.397}} $\pm$ 0.2165 \\
			& $(1, 0.1, 50)$ & 0.980 $\pm$ 0.0005 & \underline{0.943} $\pm$ 0.0005 & \underline{1.839} $\pm$ 0.0662 & \underline{0.941} $\pm$ 0.0005 & \underline{3.421} $\pm$ 0.0619 & \underline{0.936} $\pm$ 0.0005 & \underline{3.917} $\pm$ 0.1691 \\ \hline
			%
			\multirow{4}{0.10\linewidth}{Mahala-\\nobis} 
			& $(0, 0, 0)$ & 0.990 $\pm$ 0.0007 & 0.715 $\pm$ 0.0011 & 0.571 $\pm$ 0.0110 & 0.736 $\pm$ 0.0011 & 0.822 $\pm$ 0.0165 & 0.591 $\pm$ 0.0011 & 0.564 $\pm$ 0.0203 \\
			& $(0.1, 0.1, 0)$ & \underline{\textbf{0.994}} $\pm$ 0.0004 & \underline{0.950} $\pm$ 0.0009 & 1.532 $\pm$ 0.0351 & \underline{0.960} $\pm$ 0.0010 & 2.276 $\pm$ 0.0466 & \underline{0.938} $\pm$ 0.0004 & 2.915 $\pm$ 0.1132\\
			& $(0, 0, 50)$ & 0.985 $\pm$ 0.0004 & 0.880 $\pm$ 0.0005 & \underline{2.550} $\pm$ 0.0681 & 0.883 $\pm$ 0.0006 & \underline{4.091} $\pm$ 0.1013 & 0.774 $\pm$ 0.0007 & \underline{4.274} $\pm$ 0.2305\\
			& $(0.1, 0.1, 50)$ & \underline{0.992} $\pm$ 0.0006 & \underline{\textbf{0.961}} $\pm$ 0.0005 & \underline{\textbf{2.616}} $\pm$ 0.0857 & \underline{\textbf{0.966}} $\pm$ 0.0005 & \underline{\textbf{4.325}} $\pm$ 0.0055 & \underline{\textbf{0.949}} $\pm$ 0.0003 & \underline{\textbf{4.308}} $\pm$ 0.2011 \\ \bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption[]{
	\small \textbf{Results of concept learning with different parameter settings across various OOD detectors and test OOD datasets.} 
	The ID dataset is AwA for both training and test, and the auxiliary OOD dataset is MSCOCO.
% 	$\bfC'$ denotes a set of concepts discovered by baseline \citep{yeh2020completeness} (\ie $\lambda_\textrm{mse} = 0, \lambda_\textrm{norm} = 0, \lambda_\textrm{sep} = 0$).
	Hyperparameters are in the order of $(\lambda_\textrm{mse}, \lambda_\textrm{norm}, \lambda_\textrm{sep})$, and their values are set based on the scale of corresponding regularization terms in Eqn. (\ref{equ: concept learning}), for a specific choice of the OOD detector. Further investigation, including an ablation study on each regularization term can be found in Appendix \ref{sec:appendix-concept-learning-ablation}.
% 	Larger values are better for all the metrics. 
	Across the rows (for a given OOD detector and OOD dataset), the best value is \textbf{boldfaced}, and second best value is \underline{underscored}.
	The $95\%$ confidence intervals are estimated by bootstrapping the test set over $200$ trials.
% 	\textbf{Bold} numbers indicate the best results (across the rows) for a given OOD detection method and dataset. 
	%Note that by definition of $J_{\textrm{sep}}(\bfC, \bfC')$ (Eqn. \ref{eq:relative-separability}), the relative concept separability of the baseline~\citep{yeh2020completeness} is always $0$, \ie $J_{\textrm{sep}}(\bfC', \bfC') = 0$.
	}
	\label{tab:concept-learning-results}
\vspace{-.2in}
\end{table*}




% \subsection{Results}\label{subsec:results}
\subsection{Effectiveness of Our Method}
In this subsection, we carry out experiments to answer the following question: \textit{does our concept learning objective effectively encourage concepts to have the desired properties of detection completeness and concept separability?}
%
% In this subsection, we elaborate on the experiments to answer the first question (Q1) on the effectiveness of our concept learning objective.
Table~\ref{tab:concept-learning-results} summarizes the results of concept learning with various combinations of hyperparameters for the proposed regularization terms in Eqn. (\ref{equ: concept learning}): \textbf{i)} all the hyperparameters are set to $0$ (first row); \textbf{ii)} only the terms directly relevant to detection completeness (\ie reconstruction error $J_{\textrm{norm}}(\bfC, \bfg)$ and mean-squared error $J_{\textrm{mse}}(\bfC, \bfg)$) are included (second row); \textbf{iii)} only the term responsible for concept separability $J_{\textrm{sep}}(\bfC)$ is included (third row); \textbf{iv)} all the regularization terms are included (fourth row).

% We test how effectively our regularization terms improve detection completeness and concept separability, without sacrificing the classification completeness.
In all cases, we observe that the baseline achieves a high enough classification completeness score, but the lowest detection completeness and concept separability.
This indicates that the {\em concepts discovered by \citep{yeh2020completeness} would be sufficient to describe the DNN classifier, but using the same set of concepts would be inappropriate for the OOD detector.}
% We also observe that concept separability regularization term $J_{\textrm{sep}}(\bfC) > 0$ improves the relative concept separability, and when brought together with $J_{\textrm{norm}}(\bfC, \bfg)$ and  $J_{\textrm{mse}}(\bfC, \bfg) = 0$, can improve the detection completeness even further.
% By having $\lambda_\textrm{mse} > 0, \lambda_\textrm{norm} > 0, \lambda_\textrm{sep} = 0$, we observe that $\eta^{}_{\bff, S}(\bfC)$ is always improved by large margin compared to baseline.
%
% We observe that the relative concept separability $J_{\textrm{sep}}(\bfC, \bfC')$ is largest most often for the setting where $\lambda_\textrm{mse} = \lambda_\textrm{norm} = 0, \text{ and } \lambda_\textrm{sep} > 0$ (third row).
% However, the detection completeness does not improve and in some cases drops compared to the baseline setting, suggesting that there is a tradeoff between maximizing the detection completeness and concept separability.
%
In contrast, our method significantly improves the detection completeness (and even the classification completeness) by having $\lambda_\textrm{mse} > 0, \lambda_\textrm{norm} > 0$ and concept separability by having $\lambda_\textrm{sep} > 0$, compared to the baseline.
% In accordance with our design intention, our $\ell_2$ norm-based regularization and MSE regularization not only improve the detection completeness by large margin, but also the classification completeness even further.
Moreover, the three terms make the best synergy together in almost all cases.
% \jihye{For instance, given the ODIN detector and the \texttt{SUN} dataset, including our proposed regularization terms improves the detection completeness of concepts from $0.869$ to $0.969$, and the relative concept separability is increased by $0.356$, compared to when concepts are learned without the regularization terms.}
% In this setting, there is a slight decrease the relative concept separability compared to the case where only the regularization term $J_{\textrm{sep}}(\bfC)$ is included (third row). In other words, there is a tradeoff wherein we may have to sacrifice the concept separability a little in order to achieve the best possible detection completeness.

\iffalse
\mypara{Choice of Hyperparameters.}
\label{sec:hyperparameter}
In Table \ref{tab:concept-learning-results}, we set the values of $\lambda_{\textrm{norm}}, \lambda_{\textrm{mse}}$ and $\lambda_{\textrm{sep}}$ based on the scale of corresponding regularization terms in Eqn. (\ref{equ: concept learning}) (\ie $J_{\textrm{norm}}(\bfC, \bfg),  J_{\textrm{mse}}(\bfC, \bfg)$ and $ J_{\textrm{sep}}(\bfC)$, respectively) for a specific choice of the OOD detector.
Further investigation including an ablation study on each regularization term can be found in Appendix \ref{sec:appendix-concept-learning-ablation}.
From the ablation study, we note that there is a trade-off between concept separability and coherency (defined in Eqn. \ref{eq:coherency}).
This implies that high concept separability ensures easily distinguishable score patterns between detected-ID and detected-OOD inputs, but the discovered concepts may not be understandable to humans, hence the user needs to balance the degree of $\lambda_{\textrm{sep}}$ depending on the application of interest. 
\fi
% Interestingly, we observe that the concepts targeted for a particular type of OOD detector can also be applied to different types of OOD detectors (\ie the learned concepts exhibit transferability). 
% Transferability of concepts across different OOD detectors is also discussed in Appendix \ref{sec:appendix-concept-learning-transfer}.
\iffalse
\begin{figure}[h]
\centering
\subfigure{\includegraphics[width=0.31\textwidth]{figures/distr_msp_target.jpg}} 
\subfigure{\includegraphics[width=0.31\textwidth]{figures/distr_msp_yeh.jpg}} 
\subfigure{\includegraphics[width=0.31\textwidth]{figures/distr_msp_ours.jpg}} 
\caption{\textbf{Detection completeness and estimated density of OOD score $S(\bfx, \bff)$ from MSP detector.}
\textbf{Left}: Target distribution of $S(\bfx, \bff)$ in the canonical world. 
\textbf{Mid}: Distribution of $\Scon(\bfx, \bff)$ in the concept world, using concepts learned by \citep{yeh2020completeness} ($\,\lambda_\textrm{mse} = \lambda_\textrm{norm} = \lambda_\textrm{sep} = 0$).
\textbf{Right}: Distribution of $\Scon(\bfx, \bff)$ in the concept world, using concepts learned by our method ($\lambda_\textrm{mse} = 10, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$). Comparison is made between AwA test set (ID; blue) vs. SUN (OOD; red).}
\label{fig:score-distribution-msp}
\end{figure}
\fi


% \subsection{Interpretability of the Learned Concepts (Q2.)}
% \subsection{Our Metrics and Interpretability (Q2.).}
% \mypara{Reconstruction of $\hat{\calZ}$.}

\mypara{Detection completeness and accurate reconstruction of $\calZ$.}
% Other than observing increased detection completeness, 
% To gain further insights on how accurately the feature representation space can be reconstructed from concept scores, 
% Fig. \ref{fig:score-distribution} compares the distribution of the OOD detector scores in the canonical world and concept world using the concepts with different level of detection completeness.
% learned by baseline and ours. 
% Taking MSP and Energy detectors as example, 
Additionally, we observe whether the proposed evaluation metrics are well-aligned with the interpretability of the resulting concept-based explanations.
In Fig. \ref{fig:score-distribution-msp}, we observe that concepts by ~\citep{yeh2020completeness} with low detection completeness ($\eta^{}_{\bff, S}(\bfC) = 0.782$ for MSP and $\eta^{}_{\bff, S}(\bfC) = 0.682$ for Energy) lead to a strong mismatch between the score distributions on both ID data and OOD data.
In contrast, concepts learned by our method with high detection completeness ($\eta^{}_{\bff, S}(\bfC) = 0.961$ for the MSP detector, and $\eta^{}_{\bff, S}(\bfC) = 0.941$ for the Energy detector) approximate the target score distributions more closely on both ID data and OOD data.
% Overall, our experiments find that the proposed regularization terms reduce the performance gap (between the canonical world and concept world) of both the classifier and the OOD detector, leading to more \textit{accurate} explanations.
% This validates our hypothesis that accurate reconstruction of the feature representation space $\hat{\calZ}$ and the score functions are both crucial for closing the performance gap between the canonical world and concept world of both the classifier and the OOD detector.
By reducing the performance gap of OOD detector between canonical world and concept world, it leads to more \textit{accurate} explanations for OOD detectors.
% \begin{tcolorbox}
% {\textbf{Takeaway}: Our proposed concept learning objective can achieve high detection completeness and concept separability given various OOD detectors. By reducing the performance gap of OOD detector between canonical world and concept world, it leads to more \textit{accurate} explanations for OOD detectors.} 
% \end{tcolorbox}

\iffalse
\begin{figure}[bt]
\centering
\subfloat[Set 1 with low concept separability, detected-ID \label{fig:low_in}]{\includegraphics[width=0.45\columnwidth]{yeh_class17_AwA2_top10_detected_Energy.jpg}}
\hfill \hspace{-2mm}
\subfloat[Set 2 with high concept separability, detected-ID \label{fig:high_in}] {\includegraphics[width=0.45\columnwidth]{figures/ours_class17_AwA2_top10_detected_Energy.jpg}}\hfill\\
% \vspace{-1mm}
\subfloat[Set 1 with low concept separability, detected-OOD \label{fig:low_out}]{\includegraphics[width=0.45\columnwidth]{figures/yeh_class17_SUN_top10_detected_Energy.jpg}}\hfill
\subfloat[Set 2 with high concept separability, detected-OOD \label{fig:high_out}] {\includegraphics[width=0.45\columnwidth]{figures/ours_class17_SUN_top10_detected_Energy.jpg}}
\caption{
\small \textbf{Our concept separability metric and visual distinction in the concept score patterns.} For the class "Giraffe", we compare the concept score patterns using two different sets of concepts. \textbf{Left:} Averaged concept scores using concept set 1 (top-10 important concepts out of the concepts learned with $\,\lambda_\textrm{mse} = \lambda_\textrm{norm} = \lambda_\textrm{sep} = 0$). 
\textbf{Right:} Averaged concept scores using concept set 2 (top-10 important concepts out of the concepts learned with $\,\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 50$).
Concept importance is measured using the Shapley value of Eqn. (\ref{equ: ConceptSHAP}).
Concept separability is measured based on the presented 10 concepts from each set.
% For visualization of what each concept represents, see Appendix.
% C$i$ denotes $i$-th concept.
}
\label{fig:high_separa_interpretatbility}
\vspace{-0.10in}
% \vspace{-4mm}
\end{figure}
\fi


% Lastly, we illustrate how the concepts learned by our algorithm can be used to provide explanations for an OOD detector.
% By quantifying the contribution of each concept toward OOD detection results, we can identify the major concepts that an OOD detector relies on to make decisions. 
% \begin{itemize}
%     \item What set of the concepts is most prominent across the data detected as ID (or OOD) by $\mathcal{D}$?
%     \item What set of the concepts contribute to distinguish the ID and OOD data detected by $\mathcal{D}$?
%     \item How the change in concept score affects the $\mathcal{D}$'s detection result?
%     % \jihye{check perturbation generation in ATOM <-- permutation in concept space?}
% \end{itemize}
%

\iffalse
\begin{figure}[tb]
\vspace{-5mm}
% \begin{center}
%\includegraphics[width=0.45\textwidth]{figures/completeness.png}
% \hspace*{+.5cm} 
\includegraphics[scale=0.35]{figures/expl_dolphin.png}
% \vspace{-9mm}
\caption{
\small \textbf{Our concept-based explanations for Energy detector given AwA (ID) and SUN (OOD) inputs.} Concepts are discovered by our method with $\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 10$.
Visualized examples for each concept (with the corresponding $\textrm{SHAP}(\eta^{j}_{\bff, S}, 
    \bfc_i)$ score inside the parenthesis) are the receptive fields from $\Dinte$ with highest correlation to the corresponding concept vector $\bfc_i$ where $\langle \bfphi^{p,q}(\bfx), \bfc_i \rangle > 0.85$.
\vspace{-5mm}
}
\label{fig:expl_dolphin}
% \end{center}
\end{figure}
\fi

\begin{figure*}[t]
% \vspace{-3mm}
\centering
\includegraphics[width=0.9\textwidth]{figures/energy-collie.jpg}
\caption{\small \textbf{Concept-based explanations for Energy OOD detector using concepts by \citet{yeh2020completeness} vs. ours ($\lambda_\textrm{mse} = 1, \lambda_\textrm{norm} = 0.1, \lambda_\textrm{sep} = 10$)}. Images are randomly selected from AwA test set (ID) and \texttt{Places} (OOD), and all predicted to class ``Collie''.
ID profile shows the normal concept-score patterns for ID Collie images.
}
\label{fig:expl-energy-collie}
\vspace{-3mm}
\end{figure*}

\subsection{Concept-based Explanations for OOD Detectors}
\label{sec:expt_concept_based_explanations}
\mypara{Contribution of each concept to detection.}
The proposed concept learning algorithm learns concepts for both the classifier and OOD detector considering all the classes, and
we address the following question: \textit{how much does each concept contribute to the detection results for inputs predicted to a particular class?}.
% We address the following question: \textit{how much does each concept contribute to the OOD detection result?}
Recent works have adopted the Shapley value from Coalitional Game theory literature \citep{shapley1953value,fujimoto2006axiomatic} for scoring the importance of a feature subset towards the predictions of a model \citep{chen2018shapley,lundberg2017shapley,sundararajan2020shapley}.
Extending this idea, we modify the characteristic function of the Shapley value using our per-class detection completeness metric (Eqn. (\ref{equ: completeness-detection-perclass}) in Appendix \ref{sec:appendix-perclass-completeness}). 
The modified Shapley value of a concept $\bfc_i \in \bfC$ with respect to the predicted class $j \in [L]$ is defined as
% \vspace{-3mm}
\begin{align}
    \label{equ: ConceptSHAP}
    &\textrm{SHAP}(\eta^{j}_{\bff, S}, \bfc_i)  ~:=~ \nonumber \\
    &\sum_{\bfC' \subseteq \bfC \setminus \{\bfc_i\}} \!\!\!\frac{(m - |\bfC'| - 1)! \,|\bfC'|!}{m!} ~\big(\eta^{j}_{\bff, S}(\bfC' \cup \{\bfc_i\}) - \eta^{j}_{\bff, S}(\bfC')\big),
\end{align}
where $\bfC'$ is a subset of $\bfC$ excluding concept $\bfc_i$, and $\eta^{j}_{\bff, S}$ is the per-class detection completeness with respect to class $j$.
% A high Shapley value represents the average marginal contribution of $\bfc_i$ across all possible coalitions with all classes considered.
This Shapley value captures the average marginal contribution of concept $\bfc_i$ towards explaining the decisions of the OOD detector for inputs that are predicted into class $j$.
% To do so, we simply modify our detection completeness definition (Def. (\ref{def:completeness_detec})) into a per-class variant by considering data predicted into a specific class $j$.
% Also, $b_r = 0.5$ is the AUROC of a random detector.
% Note that for numerator we use predicted label -- don't have labels for OOD data. 
% Accordingly, we use SHAP($\eta^{j}_{\bff, S}(\bfC)$) to denote the Shapley score specific to class $j$.
% where $\eta^{}_{\bff, S}(\bfC)$ is replaced in Eqn. (\ref{equ: completeness-detection-perclass}).


Eventually, we interpret the behavior of the given OOD detector by plotting the concept score patterns with respect to the concepts ranked by the above Shapley importance score.
Figure~\ref{fig:expl-energy-collie} illustrates the generated explanations given correctly-detected inputs (ID\,/\,OOD input detected as ID\,/\,OOD; first row of figure), and incorrectly-detected inputs (ID\,/\,OOD input detected as OOD\,/\,ID; second row of figure).
Overall, we observe that the OOD detector predicts an input as ID when the concept scores show a similar pattern to the ID profile, or predicts an input as OOD when the concept score pattern is far from the ID profile.
For instance, the fourth input is OOD image from \texttt{Places} dataset but detected as ID, since its score for C54 (furry dog skin) is as high as usual ID Collie images (which is true in the image). Thus, we conclude this to be an understandable mistake by the OOD detector.

We also provide qualitative comparison between~\citet{yeh2020completeness} and our method in the resulting explanations for OOD detector.
We observe that~\citet{yeh2020completeness} fails to generate visually-distinguishable explanations between detected-ID and detected-OOD inputs.
The separation between the solid green bars and the orange bars in each figure becomes more visible in our explanations, which enables more intuitive interpretation for human users, and this reflects our design goal for concept separability.
It is also noteworthy that our concepts that are most important to distinguish ID Collie from OOD Collie (\ie C54 and C30) are more specific, and finer-grained characteristics of Collie, while~\citet{yeh2020completeness} finds concepts that are vaguely similar to the features of dog, but rather generic (\ie C43 and C29).
This is the reason we require more number of concepts to achieve detection completeness and concept separability, compared to solely considering the classification completeness~\footnote{In Figure~\ref{fig:expl-energy-collie}, after concept learning with $m = 100$ and duplicate removal, we find 44 non-redundant concepts for ~\citet{yeh2020completeness}, and 100 distinct concepts for ours.}.
% \jihye{@others: may add one more closing/concluding statement?}


\iffalse

Based on this concept importance metric, we can interpret the misbehavior of the given OOD detector.
Fig. \ref{fig:expl_dolphin} shows the averaged concept scores of top-10 important concepts for Energy detector between correctly detected-ID and -OOD inputs that are predicted to class ''Dolphin'' (namely, correct profiles).
Given a random ID input that is mis-detected into OOD by the OOD detector, we observe that its concept scores rather follow the detected-OOD profiles (or vice-versa, for OOD input mis-detected into ID); specifically, unusually low score for C1 (blue, wavy surface of the sea) and high score for C14~\footnote{We could not visualize C14 as there is no receptive fields with correlation to $\bfc_{14}$ greater than $0.85$, which confirms the trade-off between concept separability and human understandability, as discussed in Appendix \ref{sec:appendix-concept-learning-ablation}}, and it would look reasonable for the OOD detector to think the ID input with such OOD-like characteristics to be OOD. 
Such inspection of the OOD detector's mistakes could assist the practitioner in examining whether it was a reasonable mistake even for humans, or whether the OOD detector is simply unreliable. See Appendix \ref{sec:appendix-shapleys} for more examples of explanations.

More examples can be found in Appendix.
we present the top-ranked concepts along with the visualized examples that are nearest to the corresponding concept vector in Fig. \ref{fig:shap_buffalo}.
For the baseline method \citep{yeh2020completeness} (denoted ``baseline'' in Fig. \ref{fig:shap_buffalo}), the learned concepts are solely intended for reconstructing the behavior of the classifier. 
In this case, we observe from Fig. \ref{fig:shap_buffalo} that 
% a common set of concepts (\ie concepts 32, 10, and 47) are selected for interpreting both the classifier and OOD detector.
interpretation of both the classifier and OOD detector depends on a common set of concepts (\ie concepts 32, 10, and 47).
On the other hand, the concepts learned by our method focus on reconstructing the behavior of both the OOD detector and the classifier. In this case, we observe from Fig. \ref{fig:shap_buffalo} that a distinct set of important concepts are selected for classification and OOD detection.
We also observe that our method requires more concepts in order to address the decisions of both the classifier and OOD detector.
For instance, the number of concepts obtained by our method and the baseline are 78 and 53 (respectively), out of a total 100 concepts~\footnote{After removing redundant concepts for which the inner-product between the corresponding concept vector and any of the remaining concept vectors is larger than $0.95$.}.
More examples of concepts with high-ranking Shapley scores can be found in Appendix \ref{sec:appendix-explanation}.
We further investigate the attribution of such top-ranked concepts via counterfactual analysis in Appendix \ref{sec:appendix-counterfactual}.

\fi

% \mypara{Separability and interpretatbility}
% \begin{figure*}
%   \centering
%   \begin{tabular}{cc}
%     \subfloat[\label{fig:mnist}][Sampling distribution is skewed consistently for a single class (i.e. class 0)]
%     {
%     \hspace{-5mm}
%     \includegraphics[width=.49\linewidth]{mnist_class_0}} 
%     ~&~
%     \subfloat[\label{fig:asd}][Sampling distribution is skewed for the classes in turn (i.e. class 0, 1, 2, ...)]
%     {\includegraphics[width=.49\linewidth]{mnist_class_all}}
%   \end{tabular}
%   \caption{Accuracy vs training time-step in MNIST}
% \label{fig:mnist_results}
% \end{figure*}


==> contents/05_related.tex <==
\section{Related Work}
\mypara{OOD detection.}
Starting with a simple baseline for OOD detection based on the maximum softmax probability (MSP) score \cite{hendrycks2016msp}, recent studies have designed various scoring functions based on the outputs from the final or penultimate layers \cite{liang2018ODIN, devries2018learning}, or a combination of different intermediate layers of DNN model \cite{lee2018mahalanobis}.
Our general framework can be applied to these existing OOD detection methods by choosing a suitable intermediate layer for concept-based interpretation~\footnote{For instance, if an OOD detector makes decisions based on outputs from an intermediate layer $\ell$, the user can explain it using concepts that can reconstruct the feature representations from layer $\ell$, or an earlier layer.}.
To further improve the OOD uncertainty estimation, several works attempt to finetune the DNN classifier using auxiliary OOD training data \cite{hendrycks2018OE,lee2018training,chen2021atom}.
Complementary to these, our work is a post-hoc method that aims to explain an already-trained DNN model and its paired OOD detector. 
Our concept learning algorithm discovers concepts through optimization based on the feature representations from a DNN layer, without modifying the internals of the DNN or the OOD detector. \jihye{details of OOD to appendix}

\mypara{Post-hoc interpretability.}
Feature attribution is the most commonly used post-hoc explanation method that attributes the decision to local input features~\cite{baehrens2009grad, simonyan2013grad, smilkov2017smoothgrad, sundararajan2017IG}, but recent works have demonstrated its vulnerability to \eg adversarial perturbations~\cite{ghorbani2019fragile,heo2019fooling,slack2020fooling}. 
Adebayo \etal~\cite{adebayo2020debugging} also conduct experimental analyses and a human subject study to assess the effectiveness of feature attributions under various settings (including on OOD data), and show that feature attributions barely have any visual difference between ID inputs and OOD inputs.
% Through human subject study, they also illustrate that users do not find the resulting explanations to be intuitive guidance deciding whether to trust model predictions with OOD inputs. 

On the other hand, concept-based explanation is another type of interpretation method, which is designed to be better-aligned with human reasoning \cite{armstrong1983human-concepts,tenenbaum1999concept-learning} and intuition~\cite{ghorbani2019ace,zhou2018interpretable,bouchacourt2019educe,yeh2020completeness}. 
% Motivated by that human reasoning follows concept-based thinking by grouping similar examples and identifying resembled patterns across them \cite{armstrong1983human-concepts,tenenbaum1999concept-learning}, a line of works aimed to reason about model behaviors in a similar way as human thinking so that the resulting explanations would be more intuitive to humans \cite{kim2018tcav,ghorbani2019ace,zhou2018interpretable,bouchacourt2019educe}. 
A common implicit assumption in the concept-based explanation literature is {\em linear interpretability}, \ie the concepts lie in a linearly-projected subspace of intermediate DNN layer activations; our work is also based on this assumption.
While the scope of existing works is confined to explaining DNN classifiers, we extend the use of concept-based interpretability for explaining OOD detectors.
Our work is inspired by \cite{yeh2020completeness}, and we extend their concept-based explanation method for DNN classifiers to OOD detectors. As discussed in section \ref{sec:concept_learning}, the concept learning objective of \cite{yeh2020completeness} can be obtained as a special case of our concept learning objective for the hyper-parameter setting $\,\lambda_{\textrm{norm}} = \lambda_{\textrm{mse}} = \lambda_{\textrm{sep}} = 0$.


\iffalse

The most commonly used post-hoc explanation for DNN prediction is feature attribution, which attributes the decision to local input features \cite{baehrens2009grad, simonyan2013grad, smilkov2017smoothgrad, sundararajan2017IG}. 
% Notwithstanding the wide adoption of feature attribution to various applications \cite{}, 
Recent works have demonstrated that feature attributions are vulnerable \cite{ghorbani2019fragile,heo2019fooling,slack2020fooling}. 
\citeauthor{adebayo2020debugging} also conducts experimental analysis and human subject study to assess the effectiveness of feature attributions under various settings including OOD data, and show that feature attributions barely have visual difference between ID inputs and OOD inputs.

On the other hand, concept-based explanation is another type of interpretability to globally explain how DNN model reasons.
Motivated by that human reasoning follows concept-based thinking by grouping similar examples and identifying resembled patterns across them \cite{armstrong1983human-concepts,tenenbaum1999concept-learning}, a line of works aimed to reason about model behaviors in a similar way as human thinking so that the resulting explanations would be more intuitive to humans \cite{kim2018tcav,ghorbani2019ace,zhou2018interpretable,bouchacourt2019educe}. 
A common implicit assumption in concept-based explanation literature is linear interpretability: concepts lie in the linearly projected space of intermediate DNN activations, and our work is also based on this assumption.
Yet, while the scope of existing works is only focused on only explaining DNN prediction, we extend the use of concept-based interpretability to reasoning OOD detectors.

\fi



\iffalse
There is a growing need for post-hoc explanation methods that can be applied to working high performance DNN models that are deployed to the real-world without taking interpretability into consideration during training.
Recent studies have focused on assessing the effectiveness of post-hoc explanations ranging from human-centric evaluations [2, 5] to functionally-grounded evaluations [19, 20, 21, 22, 10, 23].
Our work is in line with contributions of evaluation of explanations; albeit with an emphasis on interpreting OOD detectors.

Contrary to the great interest in achieving high OOD detection performance, there is little effort to develop methods that can effectively reason about the detection decisions.
\cite{adebayo2020debugging} suggests caution for using feature attributions \cite{baehrens2009grad, simonyan2013grad, smilkov2017smoothgrad, sundararajan2017IG} to inspect ID and OOD inputs through empirical assessment and human subject tests.
As such, our concentration is on developing a method based on human-friendly concepts.

Concept-based explanation is a type of explanation method that .... \cite{kim2018tcav, koh2020concept-bottleneck, ghorbani2019ace}.
This line of works are based on an implicit assumption that the concepts lie in low-dimensional subspaces of some intermediate DNN activations.

concept-based explanations.. regarding the assumptions that concepts \jihye{emphasize why we chose Yeh et al. as baseline of our work, out of other concept-based explanation works -- limitations of them.} \jihye{we show the inappropriateness of concept-based explanation only with \cite{yeh2020completeness}. Need to elaborate why we chose Yeh et al. as baseline of our work out of other concept-based explanation works.} \\.\\.\\our method is also post-hoc.\\. 

The gold standard for assessing the effectiveness of an explanation is a human subject study (DoshiVelez and Kim, 2017). Poursabzi-Sangdeh et al. (2018) 
\fi



==> contents/07_ack.tex <==
\begin{ack}
We would like to thank Haizhong Zheng for his valuable comments. 
This work is partially supported by the National Science Foundation (NSF) Grants
CCF-FMitF-1836978, SaTC-Frontiers-1804648, and CCF-2046710,
and ARO grant number W911NF-17-1-0405, and DARPA-GARD problem under agreement number 885000.
\end{ack}

==> contents/08_checklist.tex <==
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec:broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:setup}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Table \ref{tab:concept-learning-results}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{sec:appendix-implementation-details}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{See References}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> notes.tex <==


Out-of-distribution (OOD) detection plays a crucial role in ensuring the safe deployment of deep neural network (DNN) classifiers. %, by handling inputs that the classifier is not trained to handle. 
% While a plethora of methods have emerged to improve detection performance, a critical gap remains in interpreting their decisions in a human-friendly way.
While a plethora of methods have focused on improving the performance of OOD detectors, a critical gap remains in interpreting their decisions in a human-friendly way.
In this work, we attempt to bridge this gap by providing explanations for OOD detectors using high-level concepts.
% Motivated by the unexplored applicability of concept-based explanations to OOD detection tasks, 
We first propose two metrics for assessing the effectiveness of a particular set of concepts: 1) \textit{detection completeness}, which quantifies the sufficiency of concepts for explaining an OOD detector's decisions, and 2) \textit{concept separability}, which captures the distributional separation between in-distribution and OOD data in a projected concept space.
We then propose a general framework for learning a set of concepts that satisfy the desired properties of detection completeness and concept separability.
Using real-world images as a testing domain, we evaluate our proposed algorithm on a diverse set of popular OOD detection methods, and demonstrate which concepts prominently contribute to the detection results via a modified Shapley value-based importance score.

\jayaram{via counterfactual analysis and a modified Shapley value-based importance score.}



% Revised intro JR

It is well known that machine learning (ML) models such as a DNN classifier can yield uncertain and unreliable predictions on OOD inputs from an unknown distribution not observed by the model during training~\cite{amodei2016AISafety,goodfellow2015explaining,nguyen2015posterior}.
OOD detectors provide a line of defense against such inputs by detecting them so that the ML model can abstain from predicting on them~\cite{hendrycks2018OE,lin2021MOOD,mohseni2020self}.
Focusing on DNN classifiers, it is common for an OOD detector to be typically trained based on the intermediate and/or final layer representations of the classifier.
The detector learns by identifying layer-activation patterns that are common to normal (in-distribution) inputs and example OOD inputs.
Being a statistical model, any OOD detector makes incorrect decisions, \ie identifies in-distribution (ID) inputs as OOD (false positives), and OOD inputs as ID (false negatives).
Therefore, it is important for a human analyst to be able to understand why an OOD detector makes a certain decision, rather than have a black-box model.
Consider the example of medical diagnosis where an OOD detector often incorrectly identifies a normal MRI as being abnormal, requiring the intervention of a human analyst.
Such errors by an OOD detector without explanations can reduce the trust that an analyst may have on the decisions of the detector. 
Moreover, understanding such decisions of an OOD detector can help in making it more accurate.

% Motivated by the importance of being able to 
Recently, there has been a steadily-increasing number of works addressing the problem of learning 
OOD detectors with better performance~\textcolor{blue}{(cite)}. 
However, the problem of explaining the decisions of an OOD detector in a human-understandable way remains fairly unexplored.
On the other hand, the problem of attributing the predictions of a classifier to certain salient inputs or higher-level concepts has also received a lot of interest recently~\cite{yeh2019completeness,kim2018tcav}.


Naturally, one may consider running an existing interpretation method for machine learning models (e.g., \cite{kim2018tcav, ghorbani2019ace}) on an example input, but that is inadequate in that it fails to provide insights as to why one example is in-distribution (ID) while another is OOD.




It is well known that machine learning (ML) models can yield uncertain and unreliable predictions on out-of-distribution (OOD) inputs, \ie inputs from outside the training distribution~\citep{amodei2016AISafety,goodfellow2015explaining,nguyen2015posterior}.
% from an unknown distribution on which the model was not trained~\citep{amodei2016AISafety,goodfellow2015explaining,nguyen2015posterior}.
% The most common practice to avoid such phenomenon is to associate a detector that identifies whether an incoming input is likely to be OOD, then reject the model's decision on the OOD input \citep{hendrycks2018OE,lin2021MOOD,mohseni2020self}.
The most common line of defense in this situation is to augment the ML model (\eg a DNN classifier) with a detector that can identify and flag such inputs as OOD. The ML model can then abstain from making predictions on such inputs~\citep{hendrycks2018OE,lin2021MOOD,mohseni2020self}.







